Monoidal computer II: Normal complexity by string diagrams

In Monoidal Computer I, we introduced a categorical model of computation where the formal reasoning about computability was supported by the simple and popular diagrammatic language of string diagrams. In the present paper, we refine and extend that model of computation to support a formal complexity theory as well. This formalization brings to the foreground the concept of normal complexity measures, which allow decompositions akin to Kleene's normal form. Such measures turn out to be just those where evaluating the complexity of a program does not require substantially more resources than evaluating the program itself. The usual time and space complexity are thus normal measures, whereas the average and the randomized complexity measures are not. While the measures that are not normal provide important design time information about algorithms, and for theoretical analyses, normal measures can also be used at run time, as practical tools of computation, e.g. to set the bounds for hypothesis testing, inductive inference and algorithmic learning.

==> PIC/Eta.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:20:29 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="23.75" y-min="-17.5" y-max="21.88" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-0.62);(6.88,-0.62);(6.88,6.38);(6.88,6.38)"
%	 />
%<parallelogram p3= "(20,4.5)"
%	 p2= "(20,10.5)"
%	 p1= "(3.75,10.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,8.75);(6.88,8.75);(6.88,19.38);(6.88,19.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "baseline"
%	 fill-style= "none"
%	 anchor-point= "(23.12,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,-15.62);(16.88,-15.62);(16.88,4.38);(16.88,4.38)"
%	 />
%<parallelogram p3= "(23.75,-9.5)"
%	 p2= "(23.75,14.38)"
%	 p1= "(0,14.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,8.75);(5.62,8.75);(8.12,8.75);(8.12,8.75);(8.12,8.75);(6.88,6.25);
%	(6.88,6.25);(6.88,6.25);(5.62,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,-0.62);(4.38,-0.62);(9.38,-0.62);(9.38,-0.62);(9.38,-0.62);(6.88,-6.25);
%	(6.88,-6.25);(6.88,-6.25);(4.38,-0.62)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.75,21.88)
\psline{->}(6.88,-0.62)(6.88,6.38)
\pspolygon[](3.75,10.5)(20,10.5)(20,4.5)(3.75,4.5)
\psline{->}(6.88,8.75)(6.88,19.38)
\rput(16.25,7.5){$\ahh$}
\rput[Br](23.12,-8.75){$\aah$}
\psline{->}(16.88,-15.62)(16.88,4.38)
\pspolygon[](0,14.38)(23.75,14.38)(23.75,-9.5)(0,-9.5)
\rput(16.88,-17.5){$\eh$}
\rput(6.88,21.88){$\fh$}
\rput(6.88,-2.5){$\bhh$}
\pspolygon(5.62,8.75)
(8.12,8.75)
(6.88,6.25)(5.62,8.75)
\pspolygon(4.38,-0.62)
(9.38,-0.62)
(6.88,-6.25)(4.38,-0.62)
\end{pspicture}


==> PIC/Gamma.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:27:19 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="23.75" y-min="-17.5" y-max="21.88" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-0.62);(6.88,-0.62);(6.88,6.38);(6.88,6.38)"
%	 />
%<parallelogram p3= "(20,4.5)"
%	 p2= "(20,10.5)"
%	 p1= "(3.75,10.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,10.62);(16.88,10.62);(16.88,19.38);(16.88,19.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "baseline"
%	 fill-style= "none"
%	 anchor-point= "(23.12,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,-15.62);(16.88,-15.62);(16.88,4.38);(16.88,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-15.64);(6.88,-15.64);(6.88,-6.88);(6.88,-6.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<parallelogram p3= "(23.75,-9.5)"
%	 p2= "(23.75,14.38)"
%	 p1= "(0,14.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<parallelogram p3= "(10,-6.75)"
%	 p2= "(10,-0.75)"
%	 p1= "(3.75,-0.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,8.75);(5.62,8.75);(8.12,8.75);(8.12,8.75);(8.12,8.75);(6.88,6.25);
%	(6.88,6.25);(6.88,6.25);(5.62,8.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.75,21.88)
\psline{->}(6.88,-0.62)(6.88,6.38)
\pspolygon[](3.75,10.5)(20,10.5)(20,4.5)(3.75,4.5)
\psline{->}(16.88,10.62)(16.88,19.38)
\rput(16.88,7.5){$\ahh$}
\rput[Br](23.12,-8.75){$\aah$}
\psline{->}(16.88,-15.62)(16.88,4.38)
\psline{->}(6.88,-15.64)(6.88,-6.88)
\rput(6.88,-3.75){$\diagonal$}
\pspolygon[](0,14.38)(23.75,14.38)(23.75,-9.5)(0,-9.5)
\rput(6.88,-17.5){$\dh$}
\pspolygon[](3.75,-0.75)(10,-0.75)(10,-6.75)(3.75,-6.75)
\rput(16.88,-17.5){$\eh$}
\rput(16.88,21.88){$\fh$}
\pspolygon(5.62,8.75)
(8.12,8.75)
(6.88,6.25)(5.62,8.75)
\end{pspicture}


==> PIC/Halt.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Aug 22 18:20:55 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="23.75" y-min="-17.5" y-max="22.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-14.38);(6.88,-14.38);(6.88,-4.24);(6.88,-4.24)"
%	 />
%<parallelogram p3= "(20,-6.12)"
%	 p2= "(20,-0.12)"
%	 p1= "(3.75,-0.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,11.87);(16.88,11.87);(16.88,20);(16.88,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,-14.38);(16.88,-14.38);(16.88,-6.25);(16.88,-6.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,0);(16.88,0);(16.88,5.62);(16.88,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<parallelogram p3= "(23.75,-9.5)"
%	 p2= "(23.75,14.38)"
%	 p1= "(0,14.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<parallelogram p3= "(20,5.75)"
%	 p2= "(20,11.75)"
%	 p1= "(13.75,11.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,-1.88);(5.62,-1.88);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(6.88,-4.38);
%	(6.88,-4.38);(6.88,-4.38);(5.62,-1.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.75,22.5)
\psline{->}(6.88,-14.38)(6.88,-4.24)
\pspolygon[](3.75,-0.12)(20,-0.12)(20,-6.12)(3.75,-6.12)
\psline{->}(16.88,11.87)(16.88,20)
\rput(16.88,-3.12){$\ahh$}
\rput[l](17.5,2.5){$\aah$}
\psline{->}(16.88,-14.38)(16.88,-6.25)
\psline{->}(16.88,0)(16.88,5.62)
\rput(16.88,8.75){$\diagonal$}
\pspolygon[](0,14.38)(23.75,14.38)(23.75,-9.5)(0,-9.5)
\rput(6.88,-17.5){$\dh$}
\pspolygon[](13.75,11.75)(20,11.75)(20,5.75)(13.75,5.75)
\rput(16.88,-17.5){$\eh$}
\rput(16.88,22.5){$\fh$}
\pspolygon(5.62,-1.88)
(8.12,-1.88)
(6.88,-4.38)(5.62,-1.88)
\end{pspicture}


==> PIC/Happa.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 16:34:39 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.88" x-max="11.88" y-min="-10.62" y-max="13.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.25,-10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.25,-8.75);(1.25,-8.75);(1.25,-1.75);(1.25,-1.75)"
%	 />
%<parallelogram p3= "(11.88,-1.75)"
%	 p2= "(11.88,4.25)"
%	 fill-style= "none"
%	 p1= "(-1.88,4.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,4.38);(8.12,4.38);(8.12,12);(8.12,12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-8.75);(8.12,-8.75);(8.12,-1.75);(8.12,-1.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,-10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11.88,13.75)
\rput(1.25,-10.62){$\dh$}
\psline{->}(1.25,-8.75)(1.25,-1.75)
\pspolygon[](-1.88,4.25)(11.88,4.25)(11.88,-1.75)(-1.88,-1.75)
\psline{->}(8.12,4.38)(8.12,12)
\rput(5,1.25){$\ahh$}
\psline{->}(8.12,-8.75)(8.12,-1.75)
\rput(8.12,-10.62){$\eh$}
\rput(8.12,13.75){$\fh$}
\end{pspicture}


==> PIC/Kappa-Halt.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:46:55 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="20.62" y-min="-16.88" y-max="31.25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-0.62);(6.88,-0.62);(6.88,5.62);(6.88,5.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,20.62);(17.5,20.62);(17.5,29.38);(17.5,29.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,-0.38);(17.5,-0.38);(17.5,3.75);(17.5,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,-0.62);(3.75,-0.62);(20,-0.62);(20,-0.62);(20,-0.62);(15,-5.62);
%	(15,-5.62);(15,-5.62);(8.75,-5.62);(8.75,-5.62);(8.75,-5.62);(3.75,-0.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11.88,-14.38);(11.88,-14.38);(11.88,-5.62);(11.88,-5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<parallelogram p3= "(20,3.88)"
%	 p2= "(20,9.88)"
%	 p1= "(3.75,9.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,6.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,10);(17.5,10);(17.5,14.38);(17.5,14.38)"
%	 />
%<parallelogram p3= "(20.62,14.5)"
%	 p2= "(20.62,20.5)"
%	 p1= "(14.38,20.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\charct$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,8.12);(5.62,8.12);(8.12,8.12);(8.12,8.12);(8.12,8.12);(6.88,5.62);
%	(6.88,5.62);(6.88,5.62);(5.62,8.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20.62,31.25)
\rput(17.5,31.25){$\dh$}
\psline{->}(6.88,-0.62)(6.88,5.62)
\psline{->}(17.5,20.62)(17.5,29.38)
\psline{->}(17.5,-0.38)(17.5,3.75)
\pspolygon(3.75,-0.62)
(20,-0.62)
(15,-5.62)
(8.75,-5.62)(3.75,-0.62)
\psline{->}(11.88,-14.38)(11.88,-5.62)
\rput(11.88,-3.12){$\diagonal$}
\rput(11.88,-16.88){$\dh$}
\pspolygon[](3.75,9.88)(20,9.88)(20,3.88)(3.75,3.88)
\rput(16.88,6.88){$\ahh$}
\psline{->}(17.5,10)(17.5,14.38)
\pspolygon[](14.38,20.5)(20.62,20.5)(20.62,14.5)(14.38,14.5)
\rput(16.88,17.5){$\charct$}
\pspolygon(5.62,8.12)
(8.12,8.12)
(6.88,5.62)(5.62,8.12)
\end{pspicture}


==> PIC/Kappa.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 16:40:34 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="23.75" y-min="-16.88" y-max="25.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-0.62);(6.88,-0.62);(6.88,4.38);(6.88,4.38)"
%	 />
%<parallelogram p3= "(20,4.5)"
%	 p2= "(20,13.12)"
%	 fill-style= "none"
%	 p1= "(3.75,13.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,13.12);(17.5,13.12);(17.5,23.12);(17.5,23.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,-0.38);(17.5,-0.38);(17.5,4.38);(17.5,4.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,-0.62);(3.75,-0.62);(20,-0.62);(20,-0.62);(20,-0.62);(15,-5.62);
%	(15,-5.62);(15,-5.62);(8.75,-5.62);(8.75,-5.62);(8.75,-5.62);(3.75,-0.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11.88,-14.38);(11.88,-14.38);(11.88,-5.62);(11.88,-5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<parallelogram p3= "(23.75,-9.5)"
%	 p2= "(23.75,16.88)"
%	 fill-style= "none"
%	 p1= "(0,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.75,25.62)
\rput(17.5,25.62){$\dh$}
\psline{->}(6.88,-0.62)(6.88,4.38)
\pspolygon[](3.75,13.12)(20,13.12)(20,4.5)(3.75,4.5)
\psline{->}(17.5,13.12)(17.5,23.12)
\rput(11.88,8.75){$\ahh$}
\psline{->}(17.5,-0.38)(17.5,4.38)
\pspolygon(3.75,-0.62)
(20,-0.62)
(15,-5.62)
(8.75,-5.62)(3.75,-0.62)
\psline{->}(11.88,-14.38)(11.88,-5.62)
\rput(11.88,-3.12){$\diagonal$}
\pspolygon[](0,16.88)(23.75,16.88)(23.75,-9.5)(0,-9.5)
\rput(11.88,-16.88){$\dh$}
\end{pspicture}


==> PIC/Kleene.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Aug 22 18:20:55 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="138.12" y-min="-19.38" y-max="88.75" auto-bounding="true">
%<parallelogram p3= "(78.12,18.24)"
%	 p2= "(78.12,24.24)"
%	 p1= "(50,24.24)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.12,21.24)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(74.38,-2.49);(74.38,-2.49);(74.38,18.12);(74.38,18.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(74.38,-5.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(74.38,24.38);(74.38,24.38);(74.38,30.62);(74.38,30.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(74.38,33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(52.5,58.12);(52.5,58.12);(52.5,64.38);(52.5,64.38)"
%	 />
%<parallelogram p3= "(68.12,62.5)"
%	 p2= "(68.12,68.5)"
%	 p1= "(50.12,68.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(52.5,66.88);(52.5,66.88);(52.5,75.62);(52.5,75.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(66.25,46.25);(66.25,46.25);(66.25,62.5);(66.25,62.5)"
%	 />
%<parallelogram p3= "(78.12,73.87)"
%	 p2= "(78.12,79.87)"
%	 p1= "(50,79.87)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.12,76.87)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,65.63)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(76.25,53.13);(76.25,53.13);(76.25,73.75);(76.25,73.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(76.25,80);(76.25,80);(76.25,86.25);(76.25,86.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<parallelogram p3= "(16.25,54.38)"
%	 p2= "(16.25,68.44)"
%	 p1= "(0,68.44)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,68.75);(3.12,68.75);(3.12,75.62);(3.12,75.62)"
%	 />
%<parallelogram p3= "(28.12,73.87)"
%	 p2= "(28.12,79.87)"
%	 p1= "(0,79.87)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.12,76.87)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25.62,53.13);(25.62,53.13);(25.62,73.75);(25.62,73.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25.62,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25.62,80);(25.62,80);(25.62,86.25);(25.62,86.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25.62,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<parallelogram p3= "(120,60)"
%	 p2= "(120,79.88)"
%	 p1= "(100,79.87)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(118.12,53.13);(118.12,53.13);(118.12,60);(118.12,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.12,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(118.12,80);(118.12,80);(118.12,86.25);(118.12,86.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.12,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<parallelogram p3= "(15,7)"
%	 p2= "(15,13)"
%	 p1= "(0,13)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(7.5,13.12);(7.5,13.12);(7.5,20);(7.5,20)"
%	 />
%<parallelogram p3= "(28.12,18.25)"
%	 p2= "(28.12,24.25)"
%	 p1= "(0,24.25)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.12,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(24.38,-2.49);(24.38,-2.49);(24.38,18.12);(24.38,18.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(24.38,-5.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(24.38,24.38);(24.38,24.38);(24.38,30.62);(24.38,30.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(24.38,33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<parallelogram p3= "(106.25,10.12)"
%	 p2= "(106.25,16.12)"
%	 p1= "(100,16.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(103.12,16.25);(103.12,16.25);(103.12,20);(103.12,20)"
%	 />
%<parallelogram p3= "(128.12,18.24)"
%	 p2= "(128.12,24.24)"
%	 p1= "(100,24.24)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(123.12,21.24)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(124.38,-2.49);(124.38,-2.49);(124.38,18.12);(124.38,18.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(124.38,-5.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(124.38,24.38);(124.38,24.38);(124.38,30.62);(124.38,30.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(124.38,33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(38.12,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.12,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(138.12,69.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.12,14.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(38.12,14.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,55.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(58.75,46.25);(58.75,46.25);(73.12,46.25);(73.12,46.25);(73.12,46.25);(66.25,39.38);
%	(66.25,39.38);(66.25,39.38);(58.75,46.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,61.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\HaH$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.75,46.25);(13.75,46.25);(13.75,54.38);(13.75,54.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,46.25);(6.25,46.25);(20.62,46.25);(20.62,46.25);(20.62,46.25);(13.75,39.38);
%	(13.75,39.38);(13.75,39.38);(6.25,46.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(103.12,52.5);(103.12,52.5);(103.12,60);(103.12,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95.62,52.5);(95.62,52.5);(110,52.5);(110,52.5);(110,52.5);(103.12,45.62);
%	(103.12,45.62);(103.12,45.62);(95.62,52.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(103.12,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Bhh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(7.5,1.25);(7.5,1.25);(7.5,6.88);(7.5,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,1.25);(0,1.25);(14.38,1.25);(14.38,1.25);(14.38,1.25);(7.5,-5.62);
%	(7.5,-5.62);(7.5,-5.62);(0,1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<parallelogram p3= "(65,7)"
%	 p2= "(65,13)"
%	 p1= "(50,13)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(57.5,13.12);(57.5,13.12);(57.5,20);(57.5,20)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(57.5,1.25);(57.5,1.25);(57.5,6.88);(57.5,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,1.25);(50,1.25);(64.38,1.25);(64.38,1.25);(64.38,1.25);(57.5,-5.62);
%	(57.5,-5.62);(57.5,-5.62);(50,1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\FaH$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<parallelogram p3= "(116.25,-7.34)"
%	 p2= "(116.25,6.09)"
%	 p1= "(100,6.09)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(103.12,6.25);(103.12,6.25);(103.12,10);(103.12,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.12,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\HaH$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(113.12,-12.5);(113.12,-12.5);(113.12,-7.5);(113.12,-7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105.62,-12.5);(105.62,-12.5);(120,-12.5);(120,-12.5);(120,-12.5);(113.12,-19.38);
%	(113.12,-19.38);(113.12,-19.38);(105.62,-12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(113.12,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ht$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(103.12,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tttt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.25,22.5);(6.25,22.5);(8.75,22.5);(8.75,22.5);(8.75,22.5);(7.5,20);
%	(7.5,20);(7.5,20);(6.25,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,22.5);(56.25,22.5);(58.75,22.5);(58.75,22.5);(58.75,22.5);(57.5,20);
%	(57.5,20);(57.5,20);(56.25,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.88,22.5);(101.88,22.5);(104.38,22.5);(104.38,22.5);(104.38,22.5);(103.12,20);
%	(103.12,20);(103.12,20);(101.88,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,66.88);(51.25,66.88);(53.75,66.88);(53.75,66.88);(53.75,66.88);(52.5,64.38);
%	(52.5,64.38);(52.5,64.38);(51.25,66.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,78.12);(51.25,78.12);(53.75,78.12);(53.75,78.12);(53.75,78.12);(52.5,75.62);
%	(52.5,75.62);(52.5,75.62);(51.25,78.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,78.12);(1.88,78.12);(4.38,78.12);(4.38,78.12);(4.38,78.12);(3.12,75.62);
%	(3.12,75.62);(3.12,75.62);(1.88,78.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,58.12);(50,58.12);(55,58.12);(55,58.12);(55,58.12);(52.51,52.5);
%	(52.51,52.5);(52.51,52.5);(50,58.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(138.12,88.75)
\pspolygon[](50,24.24)(78.12,24.24)(78.12,18.24)(50,18.24)
\rput(73.12,21.24){$\ahh$}
\psline{->}(74.38,-2.49)(74.38,18.12)
\rput(74.38,-5.62){$\chh$}
\psline{->}(74.38,24.38)(74.38,30.62)
\rput(74.38,33.12){$\Lhh$}
\psline{->}(52.5,58.12)(52.5,64.38)
\pspolygon[](50.12,68.5)(68.12,68.5)(68.12,62.5)(50.12,62.5)
\psline{->}(52.5,66.88)(52.5,75.62)
\psline{->}(66.25,46.25)(66.25,62.5)
\pspolygon[](50,79.87)(78.12,79.87)(78.12,73.87)(50,73.87)
\rput(73.12,76.87){$\ahh$}
\rput(65,65.63){$\shh$}
\psline{->}(76.25,53.13)(76.25,73.75)
\rput(76.25,50){$\chh$}
\psline{->}(76.25,80)(76.25,86.25)
\rput(76.25,88.75){$\Lhh$}
\pspolygon[](0,68.44)(16.25,68.44)(16.25,54.38)(0,54.38)
\psline{->}(3.12,68.75)(3.12,75.62)
\pspolygon[](0,79.87)(28.12,79.87)(28.12,73.87)(0,73.87)
\rput(23.12,76.87){$\ahh$}
\psline{->}(25.62,53.13)(25.62,73.75)
\rput(25.62,50){$\chh$}
\psline{->}(25.62,80)(25.62,86.25)
\rput(25.62,88.75){$\Lhh$}
\pspolygon[](100,79.87)(120,79.88)(120,60)(100,59.99)
\psline{->}(118.12,53.13)(118.12,60)
\rput(118.12,50){$\chh$}
\psline{->}(118.12,80)(118.12,86.25)
\rput(118.12,88.75){$\Lhh$}
\pspolygon[](0,13)(15,13)(15,7)(0,7)
\psline{->}(7.5,13.12)(7.5,20)
\pspolygon[](0,24.25)(28.12,24.25)(28.12,18.25)(0,18.25)
\rput(23.12,21.25){$\ahh$}
\psline{->}(24.38,-2.49)(24.38,18.12)
\rput(24.38,-5.62){$\chh$}
\psline{->}(24.38,24.38)(24.38,30.62)
\rput(24.38,33.12){$\Lhh$}
\pspolygon[](100,16.12)(106.25,16.12)(106.25,10.12)(100,10.12)
\psline{->}(103.12,16.25)(103.12,20)
\pspolygon[](100,24.24)(128.12,24.24)(128.12,18.24)(100,18.24)
\rput(123.12,21.24){$\ahh$}
\psline{->}(124.38,-2.49)(124.38,18.12)
\rput(124.38,-5.62){$\chh$}
\psline{->}(124.38,24.38)(124.38,30.62)
\rput(124.38,33.12){$\Lhh$}
\rput(38.12,70){$\eqls$}
\rput(88.12,70){$\eqls$}
\rput(138.12,69.38){$\eqls$}
\rput(88.12,14.38){$\eqls$}
\rput(38.12,14.38){$\eqls$}
\rput(52.5,55.62){$\bhh$}
\pspolygon(58.75,46.25)
(73.12,46.25)
(66.25,39.38)(58.75,46.25)
\rput(66.25,43.75){$\Ht$}
\rput(8.12,61.25){$\HaH$}
\psline{->}(13.75,46.25)(13.75,54.38)
\pspolygon(6.25,46.25)
(20.62,46.25)
(13.75,39.38)(6.25,46.25)
\rput(13.75,43.75){$\Ht$}
\psline{->}(103.12,52.5)(103.12,60)
\pspolygon(95.62,52.5)
(110,52.5)
(103.12,45.62)(95.62,52.5)
\rput(103.12,50){$\Ht$}
\rput(110,70){$\Bhh$}
\psline{->}(7.5,1.25)(7.5,6.88)
\pspolygon(0,1.25)
(14.38,1.25)
(7.5,-5.62)(0,1.25)
\rput(7.5,-1.25){$\Ht$}
\pspolygon[](50,13)(65,13)(65,7)(50,7)
\psline{->}(57.5,13.12)(57.5,20)
\psline{->}(57.5,1.25)(57.5,6.88)
\pspolygon(50,1.25)
(64.38,1.25)
(57.5,-5.62)(50,1.25)
\rput(57.5,-1.25){$\Ht$}
\rput(7.5,10){$\FaH$}
\rput(57.5,10){$\Ht$}
\pspolygon[](100,6.09)(116.25,6.09)(116.25,-7.34)(100,-7.34)
\psline{->}(103.12,6.25)(103.12,10)
\rput(108.12,-0.62){$\HaH$}
\psline{->}(113.12,-12.5)(113.12,-7.5)
\pspolygon(105.62,-12.5)
(120,-12.5)
(113.12,-19.38)(105.62,-12.5)
\rput(113.12,-15){$\Ht$}
\rput(103.12,13.12){$\tttt$}
\pspolygon(6.25,22.5)
(8.75,22.5)
(7.5,20)(6.25,22.5)
\pspolygon(56.25,22.5)
(58.75,22.5)
(57.5,20)(56.25,22.5)
\pspolygon(101.88,22.5)
(104.38,22.5)
(103.12,20)(101.88,22.5)
\pspolygon(51.25,66.88)
(53.75,66.88)
(52.5,64.38)(51.25,66.88)
\pspolygon(51.25,78.12)
(53.75,78.12)
(52.5,75.62)(51.25,78.12)
\pspolygon(1.88,78.12)
(4.38,78.12)
(3.12,75.62)(1.88,78.12)
\pspolygon(50,58.12)
(55,58.12)
(52.51,52.5)(50,58.12)
\end{pspicture}


==> PIC/NNO-mult.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 11:37:58 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.26" y-min="-2.5" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(28.75,28.75);(28.75,28.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(58.75,30);(58.75,30);(41.25,30);(41.25,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(58.75,0);(58.75,0);(41.25,0);(41.25,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,5.62)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.26,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.26,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,13.12);(8.12,13.12);(28.75,1.88);(28.75,1.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.26,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(28.75,28.75)
\psline{->}(58.75,30)(41.25,30)
\psline{->}(58.75,0)(41.25,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(16.88,5.62){$\two$}
\rput(50,32.5){$\three$}
\rput(50,-2.5){$\four$}
\rput[l](36.26,15.62){$\five$}
\rput[l](66.26,15.62){$\six$}
\psline{->}(8.12,13.12)(28.75,1.88)
\end{pspicture}


==> PIC/NNO-neg.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jul 07 15:20:11 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.25" y-min="-1.25" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(31.88,28.12);(31.88,28.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.88,30);(61.88,30);(39.38,30);(39.38,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(48.12,0);(48.12,0);(38.75,0);(38.75,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,5.62)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(43.75,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35.62,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,13.12);(8.12,13.12);(31.88,1.25);(31.88,1.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,0);(61.25,0);(51.88,0);(51.88,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$I$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(56.25,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seven$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(31.88,28.12)
\psline{->}(61.88,30)(39.38,30)
\psline{->}(48.12,0)(38.75,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(16.88,5.62){$\two$}
\rput(50,32.5){$\three$}
\rput[t](43.75,-0.62){$\four$}
\rput[l](35.62,15.62){$\five$}
\rput[l](66.25,15.62){$\six$}
\psline{->}(8.12,13.12)(31.88,1.25)
\psline{->}(61.25,0)(51.88,0)
\rput(50,0){$I$}
\rput[t](56.25,-1.25){$\seven$}
\end{pspicture}


==> PIC/NNO-pred.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 16:20:35 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.25" y-min="-2.5" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(32.5,28.75);(32.5,28.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.88,30);(61.88,30);(38.75,30);(38.75,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(56.88,0);(56.88,0);(42.5,0);(42.5,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,5.62)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35.62,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,13.12);(8.12,13.12);(28.12,2.5);(28.12,2.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(32.5,28.75)
\psline{->}(61.88,30)(38.75,30)
\psline{->}(56.88,0)(42.5,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(16.88,5.62){$\two$}
\rput(50,32.5){$\three$}
\rput(48.75,-2.5){$\four$}
\rput[l](35.62,15.62){$\five$}
\rput[l](66.25,15.62){$\six$}
\psline{->}(8.12,13.12)(28.12,2.5)
\end{pspicture}


==> PIC/NNO.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 11:39:02 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.26" y-min="-2.5" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(28.75,28.75);(28.75,28.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.75,13.12);(8.75,13.12);(31.88,1.25);(31.88,1.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(58.12,30);(58.12,30);(42.5,30);(42.5,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.88,0);(61.88,0);(37.5,0);(37.5,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,6.25)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.26,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.26,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.26,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(28.75,28.75)
\psline{->}(8.75,13.12)(31.88,1.25)
\psline{->}(58.12,30)(42.5,30)
\psline{->}(61.88,0)(37.5,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(17.5,6.25){$\two$}
\rput(50,32.5){$\three$}
\rput(50,-2.5){$\four$}
\rput[l](36.26,15.62){$\five$}
\rput[l](66.26,15.62){$\six$}
\end{pspicture}


==> PIC/OWF.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:06:48 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.62" x-max="18.26" y-min="-33.75" y-max="33.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(4.37,-21.76);(4.37,-21.76);(4.37,-16.26);(4.37,-16.26)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-21.76);(15,-21.76);(15,-16.26);(15,-16.26)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(7.13,-16.26)"
%	 p2= "(7.13,-10)"
%	 p1= "(1.63,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2,-21.76);(2,-21.76);(18.26,-21.76);(18.26,-21.76);(18.26,-21.76);(13.26,-26.76);
%	(13.26,-26.76);(13.26,-26.76);(7,-26.76);(7,-26.76);(7,-26.76);(2,-21.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.12,22.5);(18.12,22.5);(1.88,22.5);(1.88,22.5);(1.88,22.5);(6.88,27.5);
%	(6.88,27.5);(6.88,27.5);(13.12,27.5);(13.12,27.5);(13.12,27.5);(18.12,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.99,27.5);(9.99,27.5);(9.99,33.13);(9.99,33.13)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(7.13,-3.12)"
%	 p2= "(7.13,3.12)"
%	 p1= "(1.63,3.12)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.74,-16.26)"
%	 p2= "(17.76,-10)"
%	 p1= "(12.25,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-10);(15,-10);(15,22.5);(15,22.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.37,3.12);(4.37,3.12);(4.37,9.38);(4.37,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(4.37,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(4.37,0.01)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(7.12,9.38)"
%	 p2= "(7.12,15.62)"
%	 p1= "(1.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,15.62);(4.38,15.62);(4.38,22.51);(4.38,22.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,-9.38);(4.38,-9.38);(4.38,-3.12);(4.38,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(4.38,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<multicurve fill-style= "none"
%	 points= "(9.99,-30.62);(9.99,-30.62);(9.99,-26.76);(9.99,-26.76)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(13.12,-30.62);(13.12,-30.62);(9.99,-33.75);(9.99,-33.75);(9.99,-33.75);(6.88,-30.62);
%	(6.88,-30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,-30.62);(6.88,-30.62);(13.12,-30.62);(13.12,-30.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\indist$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(18.26,33.13)
\psline{->}(4.37,-21.76)(4.37,-16.26)
\psline{->}(15,-21.76)(15,-16.26)
\pspolygon[](1.63,-10)(7.13,-10)(7.13,-16.26)(1.63,-16.26)
\pspolygon(2,-21.76)
(18.26,-21.76)
(13.26,-26.76)
(7,-26.76)(2,-21.76)
\pspolygon(18.12,22.5)
(1.88,22.5)
(6.88,27.5)
(13.12,27.5)(18.12,22.5)
\psline{->}(9.99,27.5)(9.99,33.13)
\pspolygon[](1.63,3.12)(7.13,3.12)(7.13,-3.12)(1.63,-3.12)
\pspolygon[](12.25,-10)(17.76,-10)(17.74,-16.26)(12.23,-16.26)
\psline{->}(15,-10)(15,22.5)
\psline{->}(4.37,3.12)(4.37,9.38)
\rput(4.37,-13.12){$\one$}
\rput(4.37,0.01){$\two$}
\rput(15,-13.12){$\four$}
\pspolygon[](1.62,15.62)(7.12,15.62)(7.12,9.38)(1.62,9.38)
\psline{->}(4.38,15.62)(4.38,22.51)
\psline{->}(4.38,-9.38)(4.38,-3.12)
\rput(4.38,12.5){$\three$}
\psline{->}(9.99,-30.62)(9.99,-26.76)
\psline[fillstyle=solid](13.12,-30.62)
(9.99,-33.75)(6.88,-30.62)
\psline(6.88,-30.62)(13.12,-30.62)
\rput(10,25){$\indist$}
\end{pspicture}


==> PIC/Phi-appl-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:27:19 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="20" y-min="-6.88" y-max="15.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-1.25);(6.88,-1.25);(6.88,5.75);(6.88,5.75)"
%	 />
%<parallelogram p3= "(20,3.88)"
%	 p2= "(20,9.88)"
%	 p1= "(3.75,9.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,10);(17.5,10);(17.5,15.62);(17.5,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,6.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,-1);(17.5,-1);(17.5,3.75);(17.5,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(4.38,-1.25);(4.38,-1.25);(9.38,-1.25);(9.38,-1.25);(9.38,-1.25);(6.88,-6.88);
%	(6.88,-6.88);(6.88,-6.88);(4.38,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,8.12);(5.62,8.12);(8.12,8.12);(8.12,8.12);(8.12,8.12);(6.88,5.62);
%	(6.88,5.62);(6.88,5.62);(5.62,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-1.25);(15,-1.25);(20,-1.25);(20,-1.25);(20,-1.25);(17.5,-6.88);
%	(17.5,-6.88);(17.5,-6.88);(15,-1.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,15.62)
\psline{->}(6.88,-1.25)(6.88,5.75)
\pspolygon[](3.75,9.88)(20,9.88)(20,3.88)(3.75,3.88)
\psline{->}(17.5,10)(17.5,15.62)
\rput(17.5,6.88){$\ahh$}
\psline{->}(17.5,-1)(17.5,3.75)
\rput(6.88,-3.75){$\bhh$}
\pspolygon(4.38,-1.25)
(9.38,-1.25)
(6.88,-6.88)(4.38,-1.25)
\rput(17.5,-3.75){$\bhh$}
\pspolygon(5.62,8.12)
(8.12,8.12)
(6.88,5.62)(5.62,8.12)
\pspolygon(15,-1.25)
(20,-1.25)
(17.5,-6.88)(15,-1.25)
\end{pspicture}


==> PIC/Phi-appl.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:08:41 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="20" y-min="-12.5" y-max="18.75" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,1.88);(6.88,1.88);(6.88,8.88);(6.88,8.88)"
%	 />
%<parallelogram p3= "(20,7)"
%	 p2= "(20,13)"
%	 p1= "(3.75,13)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,13.12);(17.5,13.12);(17.5,18.75);(17.5,18.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,2.12);(17.5,2.12);(17.5,6.88);(17.5,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,1.88);(3.75,1.88);(20,1.88);(20,1.88);(20,1.88);(15,-3.12);
%	(15,-3.12);(15,-3.12);(8.75,-3.12);(8.75,-3.12);(8.75,-3.12);(3.75,1.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11.88,-6.88);(11.88,-6.88);(11.88,-3.12);(11.88,-3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,11.25);(5.62,11.25);(8.12,11.25);(8.12,11.25);(8.12,11.25);(6.88,8.75);
%	(6.88,8.75);(6.88,8.75);(5.62,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,-6.88);(9.38,-6.88);(14.38,-6.88);(14.38,-6.88);(14.38,-6.88);(11.88,-12.5);
%	(11.88,-12.5);(11.88,-12.5);(9.38,-6.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,18.75)
\psline{->}(6.88,1.88)(6.88,8.88)
\pspolygon[](3.75,13)(20,13)(20,7)(3.75,7)
\psline{->}(17.5,13.12)(17.5,18.75)
\rput(17.5,10){$\ahh$}
\psline{->}(17.5,2.12)(17.5,6.88)
\pspolygon(3.75,1.88)
(20,1.88)
(15,-3.12)
(8.75,-3.12)(3.75,1.88)
\psline{->}(11.88,-6.88)(11.88,-3.12)
\rput(11.88,-0.62){$\diagonal$}
\rput(11.88,-9.38){$\bhh$}
\pspolygon(5.62,11.25)
(8.12,11.25)
(6.88,8.75)(5.62,11.25)
\pspolygon(9.38,-6.88)
(14.38,-6.88)
(11.88,-12.5)(9.38,-6.88)
\end{pspicture}


==> PIC/Phi-charct.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 17:02:01 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="8.12" y-min="-16.88" y-max="31.25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.75,20.62);(3.75,20.62);(3.75,29.38);(3.75,29.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.75,-14.39);(3.75,-14.39);(3.75,-3.12);(3.75,-3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,-16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<parallelogram p3= "(8.12,-2.89)"
%	 p2= "(8.12,5.39)"
%	 fill-style= "none"
%	 p1= "(-0.62,5.39)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.75,5.62);(3.75,5.62);(3.75,14.38);(3.75,14.38)"
%	 />
%<parallelogram p3= "(6.88,14.5)"
%	 p2= "(6.88,20.5)"
%	 fill-style= "none"
%	 p1= "(0.62,20.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\charct$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(8.12,31.25)
\rput(3.75,31.25){$\dh$}
\psline{->}(3.75,20.62)(3.75,29.38)
\psline{->}(3.75,-14.39)(3.75,-3.12)
\rput(3.75,-16.88){$\dh$}
\pspolygon[](-0.62,5.39)(8.12,5.39)(8.12,-2.89)(-0.62,-2.89)
\rput(3.75,1.25){$\ahh$}
\psline{->}(3.75,5.62)(3.75,14.38)
\pspolygon[](0.62,20.5)(6.88,20.5)(6.88,14.5)(0.62,14.5)
\rput(3.12,17.5){$\charct$}
\end{pspicture}


==> PIC/Phi.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:00:46 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="23.75" y-min="-16.88" y-max="21.25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.88,-0.62);(6.88,-0.62);(6.88,6.38);(6.88,6.38)"
%	 />
%<parallelogram p3= "(20,4.5)"
%	 p2= "(20,10.5)"
%	 p1= "(3.75,10.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,10.62);(17.5,10.62);(17.5,19.38);(17.5,19.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "baseline"
%	 fill-style= "none"
%	 anchor-point= "(23.12,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17.5,-0.38);(17.5,-0.38);(17.5,4.38);(17.5,4.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,-0.62);(3.75,-0.62);(20,-0.62);(20,-0.62);(20,-0.62);(15,-5.62);
%	(15,-5.62);(15,-5.62);(8.75,-5.62);(8.75,-5.62);(8.75,-5.62);(3.75,-0.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11.88,-14.38);(11.88,-14.38);(11.88,-5.62);(11.88,-5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<parallelogram p3= "(23.75,-9.5)"
%	 p2= "(23.75,14.38)"
%	 p1= "(0,14.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,-16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.62,8.75);(5.62,8.75);(8.12,8.75);(8.12,8.75);(8.12,8.75);(6.88,6.25);
%	(6.88,6.25);(6.88,6.25);(5.62,8.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.75,21.25)
\rput(17.5,21.25){$\dh$}
\psline{->}(6.88,-0.62)(6.88,6.38)
\pspolygon[](3.75,10.5)(20,10.5)(20,4.5)(3.75,4.5)
\psline{->}(17.5,10.62)(17.5,19.38)
\rput(17.5,7.5){$\ahh$}
\rput[Br](23.12,-8.75){$\aah$}
\psline{->}(17.5,-0.38)(17.5,4.38)
\pspolygon(3.75,-0.62)
(20,-0.62)
(15,-5.62)
(8.75,-5.62)(3.75,-0.62)
\psline{->}(11.88,-14.38)(11.88,-5.62)
\rput(11.88,-3.12){$\diagonal$}
\pspolygon[](0,14.38)(23.75,14.38)(23.75,-9.5)(0,-9.5)
\rput(11.88,-16.88){$\dh$}
\pspolygon(5.62,8.75)
(8.12,8.75)
(6.88,6.25)(5.62,8.75)
\end{pspicture}


==> PIC/TDF-open.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:34:05 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="28.88" y-min="-33.75" y-max="33.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,-21.76);(15,-21.76);(15,-16.26);(15,-16.26)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-21.76);(25.62,-21.76);(25.62,-16.26);(25.62,-16.26)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-16.26)"
%	 p2= "(17.76,-10)"
%	 p1= "(12.25,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.62,-21.76);(12.62,-21.76);(28.88,-21.76);(28.88,-21.76);(28.88,-21.76);(23.88,-26.76);
%	(23.88,-26.76);(23.88,-26.76);(17.62,-26.76);(17.62,-26.76);(17.62,-26.76);(12.62,-21.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.74,22.5);(28.74,22.5);(12.5,22.5);(12.5,22.5);(12.5,22.5);(17.5,27.5);
%	(17.5,27.5);(17.5,27.5);(23.74,27.5);(23.74,27.5);(23.74,27.5);(28.74,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,27.5);(20.62,27.5);(20.62,33.13);(20.62,33.13)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-3.12)"
%	 p2= "(17.76,3.12)"
%	 p1= "(0,3.12)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(28.36,-16.26)"
%	 p2= "(28.38,-10)"
%	 p1= "(22.88,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-10);(25.62,-10);(25.62,22.5);(25.62,22.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,3.12);(15,3.12);(15,9.38);(15,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,0.01)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25.62,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(17.74,9.38)"
%	 p2= "(17.74,15.62)"
%	 p1= "(12.25,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15.62);(15,15.62);(15,22.51);(15,22.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-9.38);(15,-9.38);(15,-3.12);(15,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20.62,-30.62);(20.62,-30.62);(20.62,-26.76);(20.62,-26.76)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(23.74,-30.62);(23.74,-30.62);(20.62,-33.75);(20.62,-33.75);(20.62,-33.75);(17.5,-30.62);
%	(17.5,-30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,-30.62);(17.5,-30.62);(23.74,-30.62);(23.74,-30.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20.62,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\indist$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.12,-6.87);(3.12,-6.87);(3.12,-3.01);(3.12,-3.01)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.24,-6.87);(6.24,-6.87);(3.12,-10);(3.12,-10);(3.12,-10);(0,-6.87);
%	(0,-6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-6.87);(0,-6.87);(6.24,-6.87);(6.24,-6.87)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(22.5,-33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\exx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,-8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eyy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28.88,33.13)
\psline{->}(15,-21.76)(15,-16.26)
\psline{->}(25.62,-21.76)(25.62,-16.26)
\pspolygon[](12.25,-10)(17.76,-10)(17.76,-16.26)(12.25,-16.26)
\pspolygon(12.62,-21.76)
(28.88,-21.76)
(23.88,-26.76)
(17.62,-26.76)(12.62,-21.76)
\pspolygon(28.74,22.5)
(12.5,22.5)
(17.5,27.5)
(23.74,27.5)(28.74,22.5)
\psline{->}(20.62,27.5)(20.62,33.13)
\pspolygon[](0,3.12)(17.76,3.12)(17.76,-3.12)(0,-3.12)
\pspolygon[](22.88,-10)(28.38,-10)(28.36,-16.26)(22.85,-16.26)
\psline{->}(25.62,-10)(25.62,22.5)
\psline{->}(15,3.12)(15,9.38)
\rput(15,-13.12){$\one$}
\rput(15,0.01){$\two$}
\rput(25.62,-13.12){$\four$}
\pspolygon[](12.25,15.62)(17.74,15.62)(17.74,9.38)(12.25,9.38)
\psline{->}(15,15.62)(15,22.51)
\psline{->}(15,-9.38)(15,-3.12)
\rput(15,12.5){$\three$}
\psline{->}(20.62,-30.62)(20.62,-26.76)
\psline[fillstyle=solid](23.74,-30.62)
(20.62,-33.75)(17.5,-30.62)
\psline(17.5,-30.62)(23.74,-30.62)
\rput(20.62,25){$\indist$}
\psline{->}(3.12,-6.87)(3.12,-3.01)
\psline(6.24,-6.87)
(3.12,-10)(0,-6.87)
\psline(0,-6.87)(6.24,-6.87)
\rput[tl](22.5,-33.12){$\exx$}
\rput(3.12,-8.12){$\eyy$}
\end{pspicture}


==> PIC/TDF.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:30:06 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="28.88" y-min="-33.75" y-max="33.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,-21.76);(15,-21.76);(15,-16.26);(15,-16.26)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-21.76);(25.62,-21.76);(25.62,-16.26);(25.62,-16.26)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-16.26)"
%	 p2= "(17.76,-10)"
%	 p1= "(12.25,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.62,-21.76);(12.62,-21.76);(28.88,-21.76);(28.88,-21.76);(28.88,-21.76);(23.88,-26.76);
%	(23.88,-26.76);(23.88,-26.76);(17.62,-26.76);(17.62,-26.76);(17.62,-26.76);(12.62,-21.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.74,22.5);(28.74,22.5);(12.5,22.5);(12.5,22.5);(12.5,22.5);(17.5,27.5);
%	(17.5,27.5);(17.5,27.5);(23.74,27.5);(23.74,27.5);(23.74,27.5);(28.74,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,27.5);(20.62,27.5);(20.62,33.13);(20.62,33.13)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-3.12)"
%	 p2= "(17.76,3.12)"
%	 p1= "(0,3.12)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(28.36,-16.26)"
%	 p2= "(28.38,-10)"
%	 p1= "(22.88,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-10);(25.62,-10);(25.62,22.5);(25.62,22.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,3.12);(15,3.12);(15,9.38);(15,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,0.01)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25.62,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(17.74,9.38)"
%	 p2= "(17.74,15.62)"
%	 p1= "(12.25,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15.62);(15,15.62);(15,22.51);(15,22.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-9.38);(15,-9.38);(15,-3.12);(15,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20.62,-30.62);(20.62,-30.62);(20.62,-26.76);(20.62,-26.76)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(23.74,-30.62);(23.74,-30.62);(20.62,-33.75);(20.62,-33.75);(20.62,-33.75);(17.5,-30.62);
%	(17.5,-30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,-30.62);(17.5,-30.62);(23.74,-30.62);(23.74,-30.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20.62,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\indist$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.12,-6.87);(3.12,-6.87);(3.12,-3.01);(3.12,-3.01)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(6.24,-6.87);(6.24,-6.87);(3.12,-10);(3.12,-10);(3.12,-10);(0,-6.87);
%	(0,-6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-6.87);(0,-6.87);(6.24,-6.87);(6.24,-6.87)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(22.5,-33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\exx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(1.25,-9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eyy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28.88,33.13)
\psline{->}(15,-21.76)(15,-16.26)
\psline{->}(25.62,-21.76)(25.62,-16.26)
\pspolygon[](12.25,-10)(17.76,-10)(17.76,-16.26)(12.25,-16.26)
\pspolygon(12.62,-21.76)
(28.88,-21.76)
(23.88,-26.76)
(17.62,-26.76)(12.62,-21.76)
\pspolygon(28.74,22.5)
(12.5,22.5)
(17.5,27.5)
(23.74,27.5)(28.74,22.5)
\psline{->}(20.62,27.5)(20.62,33.13)
\pspolygon[](0,3.12)(17.76,3.12)(17.76,-3.12)(0,-3.12)
\pspolygon[](22.88,-10)(28.38,-10)(28.36,-16.26)(22.85,-16.26)
\psline{->}(25.62,-10)(25.62,22.5)
\psline{->}(15,3.12)(15,9.38)
\rput(15,-13.12){$\one$}
\rput(15,0.01){$\two$}
\rput(25.62,-13.12){$\four$}
\pspolygon[](12.25,15.62)(17.74,15.62)(17.74,9.38)(12.25,9.38)
\psline{->}(15,15.62)(15,22.51)
\psline{->}(15,-9.38)(15,-3.12)
\rput(15,12.5){$\three$}
\psline{->}(20.62,-30.62)(20.62,-26.76)
\psline[fillstyle=solid](23.74,-30.62)
(20.62,-33.75)(17.5,-30.62)
\psline(17.5,-30.62)(23.74,-30.62)
\rput(20.62,25){$\indist$}
\psline{->}(3.12,-6.87)(3.12,-3.01)
\psline[fillstyle=solid](6.24,-6.87)
(3.12,-10)(0,-6.87)
\psline(0,-6.87)(6.24,-6.87)
\rput[tl](22.5,-33.12){$\exx$}
\rput[tr](1.25,-9.38){$\eyy$}
\end{pspicture}


==> PIC/Upsilon.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 29 00:10:15 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="11.88" y-min="-12.5" y-max="19.38" auto-bounding="true">
%<parallelogram p3= "(11.88,-1.56)"
%	 p2= "(11.88,9.06)"
%	 p1= "(0,9.06)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,9.38);(3.12,9.38);(3.12,16.88);(3.12,16.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(9.38,-10);(9.38,-10);(9.38,-1.87);(9.38,-1.87)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.62,3.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\HaH$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,-12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,19.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11.88,19.38)
\pspolygon[](0,9.06)(11.88,9.06)(11.88,-1.56)(0,-1.56)
\psline{->}(3.12,9.38)(3.12,16.88)
\psline{->}(9.38,-10)(9.38,-1.87)
\rput(5.62,3.75){$\HaH$}
\rput(9.38,-12.5){$\chh$}
\rput(3.12,19.38){$\chh$}
\end{pspicture}


==> PIC/abstraction-context.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:47:10 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="17.5" y-min="-11.88" y-max="13.12" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(17.5,-1.12)"
%	 p2= "(17.5,4.88)"
%	 p1= "(1.88,4.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,3.12);(5,3.12);(5,13.12);(5,13.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.38,-11.88);(14.38,-11.88);(14.38,-1.25);(14.38,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15.62,-4.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.75,3.12);(3.75,3.12);(6.25,3.12);(6.25,3.12);(6.25,3.12);(5,0.62);
%	(5,0.62);(5,0.62);(3.75,3.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.49,-6.25);(2.49,-6.25);(7.49,-6.25);(7.49,-6.25);(7.49,-6.25);(5,-11.88);
%	(5,-11.88);(5,-11.88);(2.49,-6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.5,13.12)
\psline{->}(5,-6.25)(5,0.75)
\pspolygon[](1.88,4.88)(17.5,4.88)(17.5,-1.12)(1.88,-1.12)
\psline{->}(5,3.12)(5,13.12)
\rput(13.75,1.88){$\ahh$}
\rput(5,-8.75){$\aah$}
\psline{->}(14.38,-11.88)(14.38,-1.25)
\rput[l](15.62,-4.38){$\dh$}
\rput[r](3.75,8.12){$\dh$}
\rput[r](3.75,-3.75){$\dh$}
\pspolygon(3.75,3.12)
(6.25,3.12)
(5,0.62)(3.75,3.12)
\pspolygon(2.49,-6.25)
(7.49,-6.25)
(5,-11.88)(2.49,-6.25)
\end{pspicture}


==> PIC/abstraction.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 12:26:01 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.27" x-max="17.5" y-min="-12.5" y-max="11.88" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(17.5,-1.12)"
%	 p2= "(17.5,4.88)"
%	 fill-style= "none"
%	 p1= "(1.88,4.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,4.88);(5,4.88);(5,11.88);(5,11.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10.62,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(6,0.75)"
%	 p2= "(6,2.75)"
%	 fill-style= "solid"
%	 p1= "(4,2.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.27,-6.25);(1.27,-6.25);(8.12,-6.25);(8.12,-6.25);(8.12,-6.25);(4.39,-12.5);
%	(4.39,-12.5);(4.39,-12.5);(1.27,-6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.5,11.88)
\psline{->}(5,-6.25)(5,0.75)
\pspolygon[](1.88,4.88)(17.5,4.88)(17.5,-1.12)(1.88,-1.12)
\psline{->}(5,4.88)(5,11.88)
\rput(10.62,1.88){$\ahh$}
\rput(5,-8.75){$\aah$}
\pspolygon[fillstyle=solid](4,2.75)(6,2.75)(6,0.75)(4,0.75)
\pspolygon(1.27,-6.25)
(8.12,-6.25)
(4.39,-12.5)(1.27,-6.25)
\end{pspicture}


==> PIC/application.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 13:10:23 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.27" x-max="20.49" y-min="-12.5" y-max="11.75" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(20,-1.25)"
%	 p2= "(20,4.75)"
%	 fill-style= "none"
%	 p1= "(2,4.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,4.75);(17,4.75);(17,11.75);(17,11.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(6,0.75)"
%	 p2= "(6,2.75)"
%	 fill-style= "solid"
%	 p1= "(4,2.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,-6.25);(16.88,-6.25);(16.88,-1.25);(16.88,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.27,-6.25);(1.27,-6.25);(8.12,-6.25);(8.12,-6.25);(8.12,-6.25);(4.39,-12.5);
%	(4.39,-12.5);(4.39,-12.5);(1.27,-6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.64,-6.25);(13.64,-6.25);(20.49,-6.25);(20.49,-6.25);(20.49,-6.25);(16.76,-12.5);
%	(16.76,-12.5);(16.76,-12.5);(13.64,-6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20.49,11.75)
\psline{->}(5,-6.25)(5,0.75)
\pspolygon[](2,4.75)(20,4.75)(20,-1.25)(2,-1.25)
\psline{->}(17,4.75)(17,11.75)
\rput(13.12,1.88){$\ahh$}
\rput(5,-8.75){$\aah$}
\pspolygon[fillstyle=solid](4,2.75)(6,2.75)(6,0.75)(4,0.75)
\psline{->}(16.88,-6.25)(16.88,-1.25)
\rput(16.88,-8.75){$\bhh$}
\pspolygon(1.27,-6.25)
(8.12,-6.25)
(4.39,-12.5)(1.27,-6.25)
\pspolygon(13.64,-6.25)
(20.49,-6.25)
(16.76,-12.5)(13.64,-6.25)
\end{pspicture}


==> PIC/charfun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 23:40:21 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="55.62" y-min="-17.5" y-max="16.88" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\One$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55.62,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Five$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,11.88);(5,11.88);(5,-12.5);(5,-12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(35,11.88);(35,11.88);(35,-12.5);(35,-12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(9.38,15);(9.38,15);(31.88,15);(31.88,15)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.75,-15);(8.75,-15);(30.62,-15);(30.62,-15)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(37.5,13.12);(37.5,13.12);(51.25,2.5);(51.25,2.5)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(37.5,-12.5);(37.5,-12.5);(50,-1.25);(50,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.12,16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.75,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(29.38,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.88,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,-9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\five$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(55.62,16.88)
\rput(5,15){$\One$}
\rput(5,-15){$\Two$}
\rput(35,15){$\Three$}
\rput(35,-15){$\Four$}
\rput(55.62,0){$\Five$}
\psline{->}(5,11.88)(5,-12.5)
\psline{->}(35,11.88)(35,-12.5)
\psline{->}(9.38,15)(31.88,15)
\psline{->}(8.75,-15)(30.62,-15)
\psline{->}(37.5,13.12)(51.25,2.5)
\psline{<-}(37.5,-12.5)(50,-1.25)
\rput(18.12,16.88){$\one$}
\rput(18.75,-17.5){$\two$}
\rput(29.38,0){$\three$}
\rput(46.88,10){$\four$}
\rput(47.5,-9.38){$\five$}
\end{pspicture}


==> PIC/commutative.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 23 23:38:50 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="119" y-min="-0" y-max="26" auto-bounding="true">
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(15,16);(15,16);(15,-0);(15,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(17,16);(17,16);(5,16);(5,16);(5,16);(8,20);
%	(8,20);(8,20);(14,20);(14,20);(14,20);(17,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(11,20);(11,20);(11,26);(11,26)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(41,16);(41,16);(29,16);(29,16);(29,16);(32,20);
%	(32,20);(32,20);(38,20);(38,20);(38,20);(41,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(35,20);(35,20);(35,26);(35,26)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,18)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(11,18)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(7,16);(7,16);(7,0);(7,0)"
%	 />
%<multicurve stroke-width= "0.25"
%	 fill-style= "none"
%	 points= "(31,16);(31,16);(31,12);(32,11);(33,10);(35,9);
%	(35,9);(35,9);(37,8);(38,6);(39,4);(39,0);
%	(39,0)"
%	 />
%<multicurve stroke-width= "0.25"
%	 fill-style= "none"
%	 points= "(39,16);(39,16);(39,12);(38,11);(37,10);(35,9);
%	(35,9);(35,9);(33,8);(32,6);(31,4);(31,0);
%	(31,0)"
%	 />
%<ellipse p3= "(36,8)"
%	 p2= "(36,10)"
%	 fill-color= "#ffffff"
%	 p1= "(34,10)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,9)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\simmetry$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(80,10);(80,10);(80,26);(80,26)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(78,10);(78,10);(90,10);(90,10);(90,10);(87,6);
%	(87,6);(87,6);(81,6);(81,6);(81,6);(78,10)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(84,6);(84,6);(84,0);(84,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(107,10);(107,10);(119,10);(119,10);(119,10);(116,6);
%	(116,6);(116,6);(110,6);(110,6);(110,6);(107,10)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(113,6);(113,6);(113,0);(113,0)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(88,10);(88,10);(88,26);(88,26)"
%	 />
%<multicurve stroke-width= "0.25"
%	 fill-style= "none"
%	 points= "(117,10);(117,10);(117,14);(116,15);(115,16);(113,17);
%	(113,17);(113,17);(111,18);(110,20);(109,22);(109,26);
%	(109,26)"
%	 />
%<multicurve stroke-width= "0.25"
%	 fill-style= "none"
%	 points= "(109,10);(109,10);(109,14);(110,15);(111,16);(113,17);
%	(113,17);(113,17);(115,18);(116,20);(117,22);(117,26);
%	(117,26)"
%	 />
%<ellipse p3= "(112,18)"
%	 p2= "(112,16)"
%	 fill-color= "#ffffff"
%	 p1= "(114,16)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(113,17)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\simmetry$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(113,8)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\monoidd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(84,8)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\monoidd$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(119,26)
\psline[linewidth=0.22](15,16)(15,-0)
\pspolygon[linewidth=0.22](17,16)
(5,16)
(8,20)
(14,20)(17,16)
\psline[linewidth=0.22](11,20)(11,26)
\rput(22,10){$=$}
\pspolygon[linewidth=0.22](41,16)
(29,16)
(32,20)
(38,20)(41,16)
\psline[linewidth=0.22](35,20)(35,26)
\rput(35,18){$\comonoidd$}
\rput(11,18){$\comonoidd$}
\psline[linewidth=0.22](7,16)(7,0)
\pscustom[linewidth=0.25]{\psbezier(31,16)(31,16)(31,12)(32,11)
\psbezier(33,10)(35,9)(35,9)
\psbezier(35,9)(37,8)(38,6)
\psbezier(39,4)(39,0)(39,0)
}
\pscustom[linewidth=0.25]{\psbezier(39,16)(39,16)(39,12)(38,11)
\psbezier(37,10)(35,9)(35,9)
\psbezier(35,9)(33,8)(32,6)
\psbezier(31,4)(31,0)(31,0)
}
\rput{0}(35,9){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1,-1)}
\rput(35,9){$\simmetry$}
\psline[linewidth=0.22](80,10)(80,26)
\pspolygon[linewidth=0.22](78,10)
(90,10)
(87,6)
(81,6)(78,10)
\psline[linewidth=0.22](84,6)(84,0)
\rput(100,10){$=$}
\pspolygon[linewidth=0.22](107,10)
(119,10)
(116,6)
(110,6)(107,10)
\psline[linewidth=0.22](113,6)(113,0)
\psline[linewidth=0.22](88,10)(88,26)
\pscustom[linewidth=0.25]{\psbezier(117,10)(117,10)(117,14)(116,15)
\psbezier(115,16)(113,17)(113,17)
\psbezier(113,17)(111,18)(110,20)
\psbezier(109,22)(109,26)(109,26)
}
\pscustom[linewidth=0.25]{\psbezier(109,10)(109,10)(109,14)(110,15)
\psbezier(111,16)(113,17)(113,17)
\psbezier(113,17)(115,18)(116,20)
\psbezier(117,22)(117,26)(117,26)
}
\rput{0}(113,17){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1,-1)}
\rput(113,17){$\simmetry$}
\rput(113,8){$\monoidd$}
\rput(84,8){$\monoidd$}
\end{pspicture}


==> PIC/comp-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 16:09:24 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="10.62" y-min="-6.88" y-max="22.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.88);(5,-6.88);(5,-1.24);(5,-1.24)"
%	 />
%<parallelogram p3= "(10.62,-1.12)"
%	 p2= "(10.62,4.88)"
%	 fill-style= "none"
%	 p1= "(-0.62,4.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,4.99);(5,4.99);(5,10.62);(5,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,1.76)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<parallelogram p3= "(10.62,10.75)"
%	 p2= "(10.62,16.76)"
%	 fill-style= "none"
%	 p1= "(-0.62,16.76)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,16.88);(5,16.88);(5,22.5);(5,22.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10.62,22.5)
\psline{->}(5,-6.88)(5,-1.24)
\pspolygon[](-0.62,4.88)(10.62,4.88)(10.62,-1.12)(-0.62,-1.12)
\psline{->}(5,4.99)(5,10.62)
\rput(5,1.76){$\ahh$}
\pspolygon[](-0.62,16.76)(10.62,16.76)(10.62,10.75)(-0.62,10.75)
\psline{->}(5,16.88)(5,22.5)
\rput(5,13.75){$\chh$}
\end{pspicture}


==> PIC/comp-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 16:10:09 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="10.62" y-min="-18.75" y-max="10.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-18.75);(5,-18.75);(5,-13.12);(5,-13.12)"
%	 />
%<parallelogram p3= "(10.62,-13)"
%	 p2= "(10.62,-7)"
%	 fill-style= "none"
%	 p1= "(-0.62,-7)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.88);(5,-6.88);(5,-1.25);(5,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-10.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<parallelogram p3= "(10.62,-1.12)"
%	 p2= "(10.62,4.88)"
%	 fill-style= "none"
%	 p1= "(-0.62,4.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,5);(5,5);(5,10.62);(5,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10.62,10.62)
\psline{->}(5,-18.75)(5,-13.12)
\pspolygon[](-0.62,-7)(10.62,-7)(10.62,-13)(-0.62,-13)
\psline{->}(5,-6.88)(5,-1.25)
\rput(5,-10.12){$\ahh$}
\pspolygon[](-0.62,4.88)(10.62,4.88)(10.62,-1.12)(-0.62,-1.12)
\psline{->}(5,5)(5,10.62)
\rput(5,1.88){$\chh$}
\end{pspicture}


==> PIC/computation-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 07:01:26 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="10.62" y-min="-10" y-max="10.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,-10);(5,-10);(5,-3.12);(5,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(10.62,-3.12)"
%	 p2= "(10.62,3.75)"
%	 p1= "(-0.62,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,3.75);(5,3.75);(5,10.62);(5,10.62)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10.62,10.62)
\psline{->}(5,-10)(5,-3.12)
\rput(5,0){$\ahh$}
\pspolygon[](-0.62,3.75)(10.62,3.75)(10.62,-3.12)(-0.62,-3.12)
\psline{->}(5,3.75)(5,10.62)
\end{pspicture}


==> PIC/constant.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 17:12:20 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="10" y-min="-11.25" y-max="11.88" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-11.25);(5,-11.25);(5,-5);(5,-5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,5);(5,5);(5,11.88);(5,11.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(10,5);(10,5);(10,5);(5,0);
%	(5,0);(5,0);(0,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,-5);(10,-5);(-0,-5);(-0,-5);(-0,-5);(5,-0);
%	(5,-0);(5,-0);(10,-5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,11.88)
\psline{->}(5,-11.25)(5,-5)
\rput(5,-3.12){$\ahh$}
\rput(5,3.12){$\aah$}
\psline{->}(5,5)(5,11.88)
\pspolygon(0,5)
(10,5)
(5,0)(0,5)
\pspolygon(10,-5)
(-0,-5)
(5,-0)(10,-5)
\end{pspicture}


==> PIC/convolution-equality-P-down.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 16 10:47:33 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-16.88" y-max="35.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,-4.88);(3.12,-4.88);(3.12,0.62);(3.12,0.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,6.88);(3.12,6.88);(3.12,12.5);(3.12,12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,-4.88);(13.12,-4.88);(13.12,0.62);(13.12,0.62)"
%	 />
%<parallelogram p3= "(5.88,0.62)"
%	 p2= "(5.88,6.88)"
%	 fill-style= "none"
%	 p1= "(0.38,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,-4.88);(0.12,-4.88);(16.38,-4.88);(16.38,-4.88);(16.38,-4.88);(11.38,-9.88);
%	(11.38,-9.88);(11.38,-9.88);(5.12,-9.88);(5.12,-9.88);(5.12,-9.88);(0.12,-4.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-13.75);(8.12,-13.75);(8.12,-9.88);(8.12,-9.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,12.5);(16.25,12.5);(0,12.5);(0,12.5);(0,12.5);(5,17.5);
%	(5,17.5);(5,17.5);(11.25,17.5);(11.25,17.5);(11.25,17.5);(16.25,12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,17.5);(8.12,17.5);(8.12,21.88);(8.12,21.88)"
%	 />
%<parallelogram p3= "(15.88,0.62)"
%	 p2= "(15.88,6.88)"
%	 fill-style= "none"
%	 p1= "(10.38,6.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,6.88);(13.12,6.88);(13.12,12.5);(13.12,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram p3= "(10.88,21.88)"
%	 p2= "(10.88,28.12)"
%	 fill-style= "none"
%	 p1= "(5.38,28.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,28.12);(8.12,28.12);(8.12,33.75);(8.12,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,-13.75);(11.25,-13.75);(8.12,-16.88);(8.12,-16.88);(8.12,-16.88);(5,-13.75);
%	(5,-13.75)"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(10,-16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,35.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-13.75);(5,-13.75);(11.25,-13.75);(11.25,-13.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,35.62)
\psline{->}(3.12,-4.88)(3.12,0.62)
\psline{->}(3.12,6.88)(3.12,12.5)
\psline{->}(13.12,-4.88)(13.12,0.62)
\pspolygon[](0.38,6.88)(5.88,6.88)(5.88,0.62)(0.38,0.62)
\pspolygon(0.12,-4.88)
(16.38,-4.88)
(11.38,-9.88)
(5.12,-9.88)(0.12,-4.88)
\psline{->}(8.12,-13.75)(8.12,-9.88)
\pspolygon(16.25,12.5)
(0,12.5)
(5,17.5)
(11.25,17.5)(16.25,12.5)
\psline{->}(8.12,17.5)(8.12,21.88)
\pspolygon[](10.38,6.88)(15.88,6.88)(15.88,0.62)(10.38,0.62)
\psline{->}(13.12,6.88)(13.12,12.5)
\rput(3.12,3.75){$\one$}
\rput(13.12,3.75){$\two$}
\pspolygon[](5.38,28.12)(10.88,28.12)(10.88,21.88)(5.38,21.88)
\psline{->}(8.12,28.12)(8.12,33.75)
\psline(11.25,-13.75)
(8.12,-16.88)(5,-13.75)
\rput[tl](10,-16.25){$\variable$}
\rput(8.12,25){$\defnd$}
\rput(8.12,35.62){$\Lhh$}
\psline(5,-13.75)(11.25,-13.75)
\end{pspicture}


==> PIC/convolution-equality-P-tags.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 10:27:07 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="50.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,27.5);(3.12,27.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,15.62);(13.12,15.62)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,1.25);(8.12,1.25);(8.12,5.12);(8.12,5.12)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(15.88,15.62)"
%	 p2= "(15.88,21.88)"
%	 p1= "(10.38,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,21.88);(13.12,21.88);(13.12,27.5);(13.12,27.5)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(10.88,36.88)"
%	 p2= "(10.88,43.12)"
%	 p1= "(5.38,43.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,43.12);(8.12,43.12);(8.12,48.75);(8.12,48.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,1.25);(11.25,1.25);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(5,1.25);
%	(5,1.25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(10,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,50.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,1.25);(5,1.25);(11.25,1.25);(11.25,1.25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,24.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Mu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(1.88,24.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Mu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(1.88,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lu$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,50.62)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,27.5)
\psline{->}(13.12,10.12)(13.12,15.62)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,1.25)(8.12,5.12)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,21.88)(15.88,21.88)(15.88,15.62)(10.38,15.62)
\psline{->}(13.12,21.88)(13.12,27.5)
\rput(3.12,18.75){$\one$}
\rput(13.12,18.75){$\two$}
\pspolygon[](5.38,43.12)(10.88,43.12)(10.88,36.88)(5.38,36.88)
\psline{->}(8.12,43.12)(8.12,48.75)
\psline(11.25,1.25)
(8.12,-1.88)(5,1.25)
\rput[tl](10,-1.25){$\variable$}
\rput(8.12,40){$\defnd$}
\rput(8.12,50.62){$\Lhh$}
\psline(5,1.25)(11.25,1.25)
\rput[l](13.75,24.38){$\Mu$}
\rput[l](13.75,12.5){$\Lu$}
\rput[r](1.88,24.38){$\Mu$}
\rput[r](1.88,12.5){$\Lu$}
\end{pspicture}


==> PIC/convolution-equality-P.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 18:04:49 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="50.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,27.5);(3.12,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,15.62);(13.12,15.62)"
%	 />
%<parallelogram p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,1.25);(8.12,1.25);(8.12,5.12);(8.12,5.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 />
%<parallelogram p3= "(15.88,15.62)"
%	 p2= "(15.88,21.88)"
%	 p1= "(10.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,21.88);(13.12,21.88);(13.12,27.5);(13.12,27.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram p3= "(10.88,36.88)"
%	 p2= "(10.88,43.12)"
%	 p1= "(5.38,43.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,43.12);(8.12,43.12);(8.12,48.75);(8.12,48.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,1.25);(11.25,1.25);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(5,1.25);
%	(5,1.25)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(10,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,50.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,1.25);(5,1.25);(11.25,1.25);(11.25,1.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,50.62)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,27.5)
\psline{->}(13.12,10.12)(13.12,15.62)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,1.25)(8.12,5.12)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,21.88)(15.88,21.88)(15.88,15.62)(10.38,15.62)
\psline{->}(13.12,21.88)(13.12,27.5)
\rput(3.12,18.75){$\one$}
\rput(13.12,18.75){$\two$}
\pspolygon[](5.38,43.12)(10.88,43.12)(10.88,36.88)(5.38,36.88)
\psline{->}(8.12,43.12)(8.12,48.75)
\psline(11.25,1.25)
(8.12,-1.88)(5,1.25)
\rput[tl](10,-1.25){$\variable$}
\rput(8.12,40){$\defnd$}
\rput(8.12,50.62){$\Lhh$}
\psline(5,1.25)(11.25,1.25)
\end{pspicture}


==> PIC/convolution-equality.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 17:42:50 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="50.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,27.5);(3.12,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,15.62);(13.12,15.62)"
%	 />
%<parallelogram p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-0.62);(8.12,-0.62);(8.12,5.12);(8.12,5.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 />
%<parallelogram p3= "(15.88,15.62)"
%	 p2= "(15.88,21.88)"
%	 p1= "(10.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,21.88);(13.12,21.88);(13.12,27.5);(13.12,27.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram p3= "(10.88,36.88)"
%	 p2= "(10.88,43.12)"
%	 p1= "(5.38,43.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,43.12);(8.12,43.12);(8.12,48.75);(8.12,48.75)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(11.25,1.25);(11.25,1.25);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(5,1.25);
%	(5,1.25)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(10,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,50.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,50.62)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,27.5)
\psline{->}(13.12,10.12)(13.12,15.62)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,-0.62)(8.12,5.12)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,21.88)(15.88,21.88)(15.88,15.62)(10.38,15.62)
\psline{->}(13.12,21.88)(13.12,27.5)
\rput(3.12,18.75){$\one$}
\rput(13.12,18.75){$\two$}
\pspolygon[](5.38,43.12)(10.88,43.12)(10.88,36.88)(5.38,36.88)
\psline{->}(8.12,43.12)(8.12,48.75)
\psline[linewidth=0.05,fillstyle=solid](11.25,1.25)
(8.12,-1.88)(5,1.25)
\rput[tl](10,-1.25){$\variable$}
\rput(8.12,40){$\defnd$}
\rput(8.12,50.62){$\Lhh$}
\end{pspicture}


==> PIC/convolution-oper.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 07:09:27 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.12" x-max="25.12" y-min="-21.88" y-max="22.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(7.5,-8);(7.5,-8);(7.5,-2.51);(7.5,-2.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,3.75);(7.5,3.75);(7.5,9.38);(7.5,9.38)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.49,-8);(17.49,-8);(17.49,-2.51);(17.49,-2.51)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(10.25,-2.51)"
%	 p2= "(10.25,3.75)"
%	 p1= "(4.76,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.5,-8);(4.5,-8);(20.76,-8);(20.76,-8);(20.76,-8);(15.76,-13);
%	(15.76,-13);(15.76,-13);(9.5,-13);(9.5,-13);(9.5,-13);(4.5,-8)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,-21.88);(12.5,-21.88);(12.5,-13);(12.5,-13)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,9.38);(20.62,9.38);(4.38,9.38);(4.38,9.38);(4.38,9.38);(9.38,14.38);
%	(9.38,14.38);(9.38,14.38);(15.62,14.38);(15.62,14.38);(15.62,14.38);(20.62,9.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,14.38);(12.5,14.38);(12.5,22.5);(12.5,22.5)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(20.26,-2.51)"
%	 p2= "(20.26,3.75)"
%	 p1= "(14.76,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.49,3.75);(17.49,3.75);(17.49,9.38);(17.49,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.49,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(25.12,-17.5)"
%	 p2= "(25.12,17.5)"
%	 p1= "(-0.12,17.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "bottom"
%	 anchor-point= "(24.38,-16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ahh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(25.12,22.5)
\psline{->}(7.5,-8)(7.5,-2.51)
\psline{->}(7.5,3.75)(7.5,9.38)
\psline{->}(17.49,-8)(17.49,-2.51)
\pspolygon[](4.76,3.75)(10.25,3.75)(10.25,-2.51)(4.76,-2.51)
\pspolygon(4.5,-8)
(20.76,-8)
(15.76,-13)
(9.5,-13)(4.5,-8)
\psline{->}(12.5,-21.88)(12.5,-13)
\pspolygon(20.62,9.38)
(4.38,9.38)
(9.38,14.38)
(15.62,14.38)(20.62,9.38)
\psline{->}(12.5,14.38)(12.5,22.5)
\pspolygon[](14.76,3.75)(20.26,3.75)(20.26,-2.51)(14.76,-2.51)
\psline{->}(17.49,3.75)(17.49,9.38)
\rput(7.5,0.62){$\one$}
\rput(17.49,0.62){$\two$}
\pspolygon[](-0.12,17.5)(25.12,17.5)(25.12,-17.5)(-0.12,-17.5)
\rput[br](24.38,-16.88){$\ahh$}
\end{pspicture}


==> PIC/convolution.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 23 14:38:49 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.25" y-min="0" y-max="38.75" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,11.88);(3.12,11.88);(3.12,16.86);(3.12,16.86)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,23.12);(3.12,23.12);(3.12,27.5);(3.12,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,11.88);(13.12,11.88);(13.12,16.86);(13.12,16.86)"
%	 />
%<parallelogram p3= "(5.88,16.86)"
%	 p2= "(5.88,23.12)"
%	 p1= "(0.38,23.12)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.88);(0,11.88);(16.25,11.88);(16.25,11.88);(16.25,11.88);(11.38,7);
%	(11.38,7);(11.38,7);(5.12,7);(5.12,7);(5.12,7);(0,11.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,2.5);(8.12,2.5);(8.12,7);(8.12,7)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 />
%<parallelogram p3= "(15.88,16.86)"
%	 p2= "(15.88,23.12)"
%	 p1= "(10.38,23.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,23.12);(13.12,23.12);(13.12,27.5);(13.12,27.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Source$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,38.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Target$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,38.75)
\psline{->}(3.12,11.88)(3.12,16.86)
\psline{->}(3.12,23.12)(3.12,27.5)
\psline{->}(13.12,11.88)(13.12,16.86)
\pspolygon[](0.38,23.12)(5.88,23.12)(5.88,16.86)(0.38,16.86)
\pspolygon(0,11.88)
(16.25,11.88)
(11.38,7)
(5.12,7)(0,11.88)
\psline{->}(8.12,2.5)(8.12,7)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,23.12)(15.88,23.12)(15.88,16.86)(10.38,16.86)
\psline{->}(13.12,23.12)(13.12,27.5)
\rput(3.12,20){$\one$}
\rput(13.12,20){$\two$}
\rput(8.12,0){$\Source$}
\rput(8.12,38.75){$\Target$}
\end{pspicture}


==> PIC/diag-comm <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 12 19:13:12 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="30" y-min="-2.5" y-max="16.25" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.49,2.5);(2.49,2.5);(13.75,13.75);(13.75,13.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,0);(3.75,0);(26.25,0);(26.25,0)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.88,9.38)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,9.38)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,13.75);(16.25,13.75);(27.5,2.5);(27.5,2.5)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(30,16.25)
\rput(0,0){$\Lhh$}
\rput(15,16.25){$\UpOne$}
\rput(30,0){$\DownOne$}
\psline{->}(2.49,2.5)(13.75,13.75)
\psline{->}(3.75,0)(26.25,0)
\rput{45}(6.88,9.38){$\one$}
\rput{-45}(23.12,9.38){$\two$}
\rput(13.75,-2.5){$\four$}
\psline{->}(16.25,13.75)(27.5,2.5)
\end{pspicture}


==> PIC/diag-comm.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 12 19:16:04 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="30" y-min="-2.5" y-max="16.25" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.49,2.5);(2.49,2.5);(13.75,13.75);(13.75,13.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,0);(3.75,0);(26.25,0);(26.25,0)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.88,9.38)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,9.38)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,13.75);(16.25,13.75);(27.5,2.5);(27.5,2.5)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(30,16.25)
\rput(0,0){$\Lhh$}
\rput(15,16.25){$\UpOne$}
\rput(30,0){$\DownOne$}
\psline{->}(2.49,2.5)(13.75,13.75)
\psline{->}(3.75,0)(26.25,0)
\rput{45}(6.88,9.38){$\one$}
\rput{-45}(23.12,9.38){$\two$}
\rput(13.75,-2.5){$\four$}
\psline{->}(16.25,13.75)(27.5,2.5)
\end{pspicture}


==> PIC/diag-compreh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jul 13 16:10:51 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.88" x-max="17.13" y-min="-3.12" y-max="67.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.37,10.12);(14.37,10.12);(14.37,15.62);(14.37,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.37,21.88);(14.37,21.88);(14.37,31.25);(14.37,31.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.87,10.12);(1.87,10.12);(1.88,15.62);(1.88,15.62)"
%	 />
%<parallelogram p3= "(17.13,15.62)"
%	 p2= "(17.13,21.88)"
%	 p1= "(11.63,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,0.12);(8.12,0.12);(8.12,5.12);(8.12,5.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,43.75);(16.25,43.75);(0,43.75);(0,43.75);(0,43.75);(5,48.75);
%	(5,48.75);(5,48.75);(11.25,48.75);(11.25,48.75);(11.25,48.75);(16.25,43.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,48.75);(8.12,48.75);(8.12,54.38);(8.12,54.38)"
%	 />
%<parallelogram p3= "(17.13,31.25)"
%	 p2= "(17.13,37.5)"
%	 p1= "(11.63,37.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(4.62,15.62)"
%	 p2= "(4.63,21.88)"
%	 p1= "(-0.87,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.88,21.88);(1.88,21.88);(1.87,43.75);(1.87,43.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.37,37.5);(14.37,37.5);(14.37,43.75);(14.37,43.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(0.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.62,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,63.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.37,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.37,34.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram p3= "(10.88,54.38)"
%	 p2= "(10.88,60.62)"
%	 p1= "(5.38,60.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,60.62);(8.12,60.62);(8.12,67.5);(8.12,67.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,51.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,-3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Xhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predicate$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.13,67.5)
\psline{->}(14.37,10.12)(14.37,15.62)
\psline{->}(14.37,21.88)(14.37,31.25)
\psline{->}(1.87,10.12)(1.88,15.62)
\pspolygon[](11.63,21.88)(17.13,21.88)(17.13,15.62)(11.63,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,0.12)(8.12,5.12)
\pspolygon(16.25,43.75)
(0,43.75)
(5,48.75)
(11.25,48.75)(16.25,43.75)
\psline{->}(8.12,48.75)(8.12,54.38)
\pspolygon[](11.63,37.5)(17.13,37.5)(17.13,31.25)(11.63,31.25)
\pspolygon[](-0.87,21.88)(4.63,21.88)(4.62,15.62)(-0.88,15.62)
\psline{->}(1.88,21.88)(1.87,43.75)
\psline{->}(14.37,37.5)(14.37,43.75)
\rput[r](0.62,32.5){$\Lhh$}
\rput[l](15.62,26.25){$\UpOne$}
\rput[l](9.38,63.75){$\DownOne$}
\rput(14.37,18.75){$\one$}
\rput(14.37,34.38){$\two$}
\rput(1.88,18.75){$\four$}
\pspolygon[](5.38,60.62)(10.88,60.62)(10.88,54.38)(5.38,54.38)
\psline{->}(8.12,60.62)(8.12,67.5)
\rput[l](9.38,51.25){$\Lhh$}
\rput(8.12,-3.12){$\Xhh$}
\rput(8.12,57.5){$\predicate$}
\end{pspicture}


==> PIC/diag-string.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 12 19:17:11 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="58.12" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,31.25);(3.12,31.25)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,23.75);(13.12,23.75)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,0.12);(8.12,0.12);(8.12,5.12);(8.12,5.12)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,43.75);(16.25,43.75);(0,43.75);(0,43.75);(0,43.75);(5,48.75);
%	(5,48.75);(5,48.75);(11.25,48.75);(11.25,48.75);(11.25,48.75);(16.25,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,48.75);(8.12,48.75);(8.12,55.75);(8.12,55.75)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(5.88,31.25)"
%	 p2= "(5.88,37.5)"
%	 p1= "(0.38,37.5)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(15.88,23.75)"
%	 p2= "(15.88,30)"
%	 p1= "(10.38,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,30);(13.12,30);(13.12,43.75);(13.12,43.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,37.5);(3.12,37.5);(3.12,43.75);(3.12,43.75)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0.62,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,58.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,34.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,26.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,58.12)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,31.25)
\psline{->}(13.12,10.12)(13.12,23.75)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,0.12)(8.12,5.12)
\pspolygon(16.25,43.75)
(0,43.75)
(5,48.75)
(11.25,48.75)(16.25,43.75)
\psline{->}(8.12,48.75)(8.12,55.75)
\pspolygon[](0.38,37.5)(5.88,37.5)(5.88,31.25)(0.38,31.25)
\pspolygon[](10.38,30)(15.88,30)(15.88,23.75)(10.38,23.75)
\psline{->}(13.12,30)(13.12,43.75)
\psline{->}(3.12,37.5)(3.12,43.75)
\rput(8.12,-1.88){$\Lhh$}
\rput(0.62,26.25){$\UpOne$}
\rput(8.12,58.12){$\DownOne$}
\rput(3.12,18.75){$\one$}
\rput(3.12,34.38){$\two$}
\rput(13.12,26.88){$\four$}
\end{pspicture}


==> PIC/ensemble-square.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 18 21:54:14 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="104.38" y-min="0" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "top"
%	 anchor-point= "(1.88,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(1.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(31.25,30);(31.25,30);(12,30);(12,30)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(31.25,0);(31.25,0);(12,0);(12,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.75,26.88);(3.75,26.88);(3.75,4.38);(3.75,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(33.75,26.88);(33.75,26.88);(33.75,4.38);(33.75,4.38)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,15.62)"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\six$
%</text>
%<multicurve left-arrow= "head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(101.25,30);(101.25,30);(90,30);(90,30)"
%	 />
%<multicurve left-arrow= "head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(101.25,0);(101.25,0);(89.38,0);(89.38,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(63.75,26.88);(63.75,26.88);(63.75,4.38);(63.75,4.38)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(61.88,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpThree$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(61.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownThree$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seven$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(86,30);(86,30);(72,30);(72,30)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(86,0);(86,0);(72,0);(72,0)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,30);(61.25,30);(42,30);(42,30)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,0);(61.25,0);(42,0);(42,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(100.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpFour$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(101.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownFour$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(103.12,26.87);(103.12,26.87);(103.12,4.38);(103.12,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(104.38,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eight$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(104.38,32.5)
\rput[tl](1.88,32.5){$\UpOne$}
\rput[tl](31.88,32.5){$\UpTwo$}
\rput[tl](1.88,2.5){$\DownOne$}
\psline{<-<}(31.25,30)(12,30)
\psline{<-<}(31.25,0)(12,0)
\psline{->}(3.75,26.88)(3.75,4.38)
\psline{->}(33.75,26.88)(33.75,4.38)
\rput[tl](31.88,2.5){$\DownTwo$}
\rput[r](1.88,15.62){$\five$}
\rput[r](31.88,15.62){$\six$}
\psline[linewidth=0.5,linestyle=dotted]{<-}(101.25,30)(90,30)
\psline[linewidth=0.5,linestyle=dotted]{<-}(101.25,0)(89.38,0)
\psline{->}(63.75,26.88)(63.75,4.38)
\rput[tl](61.88,32.5){$\UpThree$}
\rput[tl](61.88,2.5){$\DownThree$}
\rput[r](62.5,15){$\seven$}
\psline[linewidth=0.5,linestyle=dotted]{-<}(86,30)(72,30)
\psline[linewidth=0.5,linestyle=dotted]{-<}(86,0)(72,0)
\psline{<-<}(61.25,30)(42,30)
\psline{<-<}(61.25,0)(42,0)
\rput[tl](100.62,32.5){$\UpFour$}
\rput[tl](101.25,2.5){$\DownFour$}
\psline{->}(103.12,26.87)(103.12,4.38)
\rput[l](104.38,15){$\eight$}
\end{pspicture}


==> PIC/ensemble-tower.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 18 22:15:42 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="101.25" y-min="0" y-max="2.5" auto-bounding="true">
%<text text-vert-align= "top"
%	 anchor-point= "(1.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(31.25,0);(31.25,0);(12,0);(12,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownTwo$
%</text>
%<multicurve left-arrow= "head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(101.25,0);(101.25,0);(89.38,0);(89.38,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(61.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownThree$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(86,0);(86,0);(72,0);(72,0)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,0);(61.25,0);(42,0);(42,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(101.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownFour$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(101.25,2.5)
\rput[tl](1.88,2.5){$\DownOne$}
\psline{<-<}(31.25,0)(12,0)
\rput[tl](31.88,2.5){$\DownTwo$}
\psline[linewidth=0.5,linestyle=dotted]{<-}(101.25,0)(89.38,0)
\rput[tl](61.88,2.5){$\DownThree$}
\psline[linewidth=0.5,linestyle=dotted]{-<}(86,0)(72,0)
\psline{<-<}(61.25,0)(42,0)
\rput[tl](101.25,2.5){$\DownFour$}
\end{pspicture}


==> PIC/f.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:05:51 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="5.62" y-min="-3.13" y-max="7.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(2.49,0);(2.49,0);(2.5,7.5);(2.5,7.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,0);(5.62,0);(2.49,-3.13);(2.49,-3.13);(2.49,-3.13);(-0.62,0);
%	(-0.62,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\variable$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,0);(-0.62,0);(5.62,0);(5.62,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(5.62,7.5)
\psline{->}(2.49,0)(2.5,7.5)
\psline(5.62,0)
(2.49,-3.13)(-0.62,0)
\rput(2.5,-1.25){$\variable$}
\psline(-0.62,0)(5.62,0)
\end{pspicture}


==> PIC/fp-wide-apply-twice.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 17:22:08 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="11.25" y-min="-8.75" y-max="40" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-1.25);(5,-1.25);(5,4.38);(5,4.38)"
%	 />
%<parallelogram p3= "(10.62,4.5)"
%	 p2= "(10.62,10.5)"
%	 fill-style= "none"
%	 p1= "(-0.62,10.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,10.62);(5,10.62);(5,16.25);(5,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,-1.25);(-0.62,-1.25);(11.25,-1.25);(11.25,-1.25);(11.25,-1.25);(5,-8.75);
%	(5,-8.75);(5,-8.75);(-0.62,-1.25)"
%	 />
%<parallelogram p3= "(10.62,16.38)"
%	 p2= "(10.62,22.38)"
%	 fill-style= "none"
%	 p1= "(-0.62,22.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,22.5);(5,22.5);(5,28.12);(5,28.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<parallelogram p3= "(10.62,28.26)"
%	 p2= "(10.62,34.25)"
%	 fill-style= "none"
%	 p1= "(-0.62,34.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,34.38);(5,34.38);(5,40);(5,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dhh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11.25,40)
\psline{->}(5,-1.25)(5,4.38)
\pspolygon[](-0.62,10.5)(10.62,10.5)(10.62,4.5)(-0.62,4.5)
\psline{->}(5,10.62)(5,16.25)
\rput(5,7.38){$\ahh$}
\rput(5,-3.75){$\bhh$}
\pspolygon(-0.62,-1.25)
(11.25,-1.25)
(5,-8.75)(-0.62,-1.25)
\pspolygon[](-0.62,22.38)(10.62,22.38)(10.62,16.38)(-0.62,16.38)
\psline{->}(5,22.5)(5,28.12)
\rput(5,19.38){$\chh$}
\pspolygon[](-0.62,34.25)(10.62,34.25)(10.62,28.26)(-0.62,28.26)
\psline{->}(5,34.38)(5,40)
\rput(5,31.25){$\dhh$}
\end{pspicture}


==> PIC/fp-wide-apply.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 13:10:30 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="11.25" y-min="-8.75" y-max="28.12" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-1.25);(5,-1.25);(5,4.38);(5,4.38)"
%	 />
%<parallelogram p3= "(10.62,4.5)"
%	 p2= "(10.62,10.5)"
%	 fill-style= "none"
%	 p1= "(-0.62,10.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,10.62);(5,10.62);(5,16.25);(5,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,-1.25);(-0.62,-1.25);(11.25,-1.25);(11.25,-1.25);(11.25,-1.25);(5,-8.75);
%	(5,-8.75);(5,-8.75);(-0.62,-1.25)"
%	 />
%<parallelogram p3= "(10.62,16.38)"
%	 p2= "(10.62,22.38)"
%	 fill-style= "none"
%	 p1= "(-0.62,22.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,22.5);(5,22.5);(5,28.12);(5,28.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11.25,28.12)
\psline{->}(5,-1.25)(5,4.38)
\pspolygon[](-0.62,10.5)(10.62,10.5)(10.62,4.5)(-0.62,4.5)
\psline{->}(5,10.62)(5,16.25)
\rput(5,7.38){$\ahh$}
\rput(5,-3.75){$\bhh$}
\pspolygon(-0.62,-1.25)
(11.25,-1.25)
(5,-8.75)(-0.62,-1.25)
\pspolygon[](-0.62,22.38)(10.62,22.38)(10.62,16.38)(-0.62,16.38)
\psline{->}(5,22.5)(5,28.12)
\rput(5,19.38){$\chh$}
\end{pspicture}


==> PIC/fp-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 13:09:06 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="11.25" y-min="-8.75" y-max="16.25" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-1.25);(5,-1.25);(5,4.38);(5,4.38)"
%	 />
%<parallelogram p3= "(10.62,4.5)"
%	 p2= "(10.62,10.5)"
%	 fill-style= "none"
%	 p1= "(-0.62,10.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,10.62);(5,10.62);(5,16.25);(5,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,-1.25);(-0.62,-1.25);(11.25,-1.25);(11.25,-1.25);(11.25,-1.25);(5,-8.75);
%	(5,-8.75);(5,-8.75);(-0.62,-1.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11.25,16.25)
\psline{->}(5,-1.25)(5,4.38)
\pspolygon[](-0.62,10.5)(10.62,10.5)(10.62,4.5)(-0.62,4.5)
\psline{->}(5,10.62)(5,16.25)
\rput(5,7.38){$\ahh$}
\rput(5,-3.75){$\bhh$}
\pspolygon(-0.62,-1.25)
(11.25,-1.25)
(5,-8.75)(-0.62,-1.25)
\end{pspicture}


==> PIC/fp-wider-elt.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 15:00:30 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.25" y-min="-7.5" y-max="5.63" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,0);(8.12,0);(8.12,5.63);(8.12,5.63)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,0);(0,0);(16.25,0);(16.25,0);(16.25,0);(8.12,-7.5);
%	(8.12,-7.5);(8.12,-7.5);(0,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,5.63)
\psline{->}(8.12,0)(8.12,5.63)
\rput(8.12,-2.5){$\bhh$}
\pspolygon(0,0)
(16.25,0)
(8.12,-7.5)(0,0)
\end{pspicture}


==> PIC/fp-wider.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jul 07 18:02:59 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.24" y-min="-12.5" y-max="12.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-5);(8.12,-5);(8.12,0.63);(8.12,0.63)"
%	 />
%<parallelogram p3= "(13.74,0.75)"
%	 p2= "(13.74,6.75)"
%	 fill-style= "none"
%	 p1= "(2.5,6.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,6.87);(8.12,6.87);(8.12,12.5);(8.12,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,3.63)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,-5);(0,-5);(16.24,-5);(16.24,-5);(16.24,-5);(8.12,-12.5);
%	(8.12,-12.5);(8.12,-12.5);(0,-5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.24,12.5)
\psline{->}(8.12,-5)(8.12,0.63)
\pspolygon[](2.5,6.75)(13.74,6.75)(13.74,0.75)(2.5,0.75)
\psline{->}(8.12,6.87)(8.12,12.5)
\rput(8.12,3.63){$\ahh$}
\rput(8.12,-7.5){$\bhh$}
\pspolygon(0,-5)
(16.24,-5)
(8.12,-12.5)(0,-5)
\end{pspicture}


==> PIC/fp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:10:33 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2" x-max="8" y-min="-6.88" y-max="16.25" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-1.25);(5,-1.25);(5,4.38);(5,4.38)"
%	 />
%<parallelogram p3= "(8,4.38)"
%	 p2= "(8,10.38)"
%	 p1= "(2,10.38)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,10.38);(5,10.38);(5,16.25);(5,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,-1.25);(2.5,-1.25);(7.5,-1.25);(7.5,-1.25);(7.5,-1.25);(5,-6.88);
%	(5,-6.88);(5,-6.88);(2.5,-1.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(8,16.25)
\psline{->}(5,-1.25)(5,4.38)
\pspolygon[](2,10.38)(8,10.38)(8,4.38)(2,4.38)
\psline{->}(5,10.38)(5,16.25)
\rput(5,7.38){$\ahh$}
\rput(5,-3.75){$\bhh$}
\pspolygon(2.5,-1.25)
(7.5,-1.25)
(5,-6.88)(2.5,-1.25)
\end{pspicture}


==> PIC/inner-product-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 23 14:36:15 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.25" y-min="6.25" y-max="29.38" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10);(3.12,10);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,15.62);(16.25,15.62);(0,15.62);(0,15.62);(0,15.62);(5,20.62);
%	(5,20.62);(5,20.62);(11.25,20.62);(11.25,20.62);(11.25,20.62);(16.25,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,20.62);(8.12,20.62);(8.12,26.25);(8.12,26.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10);(13.12,10);(13.12,15.62);(13.12,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,8.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,8.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.25,26.25);(11.25,26.25);(5,26.25);(5,26.25);(5,26.25);(8.12,29.38);
%	(8.12,29.38);(8.12,29.38);(8.12,29.38);(8.12,29.38);(8.12,29.38);(11.25,26.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,10);(16.25,10);(10,10);(10,10);(10,10);(13.12,6.25);
%	(13.12,6.25);(13.12,6.25);(13.12,6.25);(13.12,6.25);(13.12,6.25);(16.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,10);(6.25,10);(0,10);(0,10);(0,10);(3.12,6.25);
%	(3.12,6.25);(3.12,6.25);(3.12,6.25);(3.12,6.25);(3.12,6.25);(6.25,10)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,29.38)
\psline{->}(3.12,10)(3.12,15.62)
\pspolygon(16.25,15.62)
(0,15.62)
(5,20.62)
(11.25,20.62)(16.25,15.62)
\psline{->}(8.12,20.62)(8.12,26.25)
\psline{->}(13.12,10)(13.12,15.62)
\rput(3.12,8.75){$\one$}
\rput(13.12,8.75){$\two$}
\pscustom[]{\psline(11.25,26.25)(5,26.25)
\psline(5,26.25)(8.12,29.38)
\psbezier(8.12,29.38)(8.12,29.38)(8.12,29.38)
\psline(8.12,29.38)(11.25,26.25)
\closepath}
\pscustom[]{\psline(16.25,10)(10,10)
\psline(10,10)(13.12,6.25)
\psbezier(13.12,6.25)(13.12,6.25)(13.12,6.25)
\psline(13.12,6.25)(16.25,10)
\closepath}
\pscustom[]{\psline(6.25,10)(0,10)
\psline(0,10)(3.12,6.25)
\psbezier(3.12,6.25)(3.12,6.25)(3.12,6.25)
\psline(3.12,6.25)(6.25,10)
\closepath}
\end{pspicture}


==> PIC/inner-product.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 23 14:42:10 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.25" y-min="6.25" y-max="27.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10);(3.12,10);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,15.62);(16.25,15.62);(0,15.62);(0,15.62);(0,15.62);(5,20.62);
%	(5,20.62);(5,20.62);(11.25,20.62);(11.25,20.62);(11.25,20.62);(16.25,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,20.62);(8.12,20.62);(8.12,24.38);(8.12,24.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10);(13.12,10);(13.12,15.62);(13.12,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,8.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,8.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.25,24.38);(11.25,24.38);(5,24.38);(5,24.38);(5,24.38);(8.12,27.5);
%	(8.12,27.5);(8.12,27.5);(8.12,27.5);(8.12,27.5);(8.12,27.5);(11.25,24.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,10);(16.25,10);(10,10);(10,10);(10,10);(13.12,6.25);
%	(13.12,6.25);(13.12,6.25);(13.12,6.25);(13.12,6.25);(13.12,6.25);(16.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,10);(6.25,10);(0,10);(0,10);(0,10);(3.12,6.25);
%	(3.12,6.25);(3.12,6.25);(3.12,6.25);(3.12,6.25);(3.12,6.25);(6.25,10)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,27.5)
\psline{->}(3.12,10)(3.12,15.62)
\pspolygon(16.25,15.62)
(0,15.62)
(5,20.62)
(11.25,20.62)(16.25,15.62)
\psline{->}(8.12,20.62)(8.12,24.38)
\psline{->}(13.12,10)(13.12,15.62)
\rput(3.12,8.75){$\one$}
\rput(13.12,8.75){$\two$}
\pscustom[]{\psline(11.25,24.38)(5,24.38)
\psline(5,24.38)(8.12,27.5)
\psbezier(8.12,27.5)(8.12,27.5)(8.12,27.5)
\psline(8.12,27.5)(11.25,24.38)
\closepath}
\pscustom[]{\psline(16.25,10)(10,10)
\psline(10,10)(13.12,6.25)
\psbezier(13.12,6.25)(13.12,6.25)(13.12,6.25)
\psline(13.12,6.25)(16.25,10)
\closepath}
\pscustom[]{\psline(6.25,10)(0,10)
\psline(0,10)(3.12,6.25)
\psbezier(3.12,6.25)(3.12,6.25)(3.12,6.25)
\psline(3.12,6.25)(6.25,10)
\closepath}
\end{pspicture}


==> PIC/lambda-s.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:33:06 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="31.88" y-min="0" y-max="38.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,5.62);(3.12,5.62);(3.12,13.75);(3.12,13.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(18.12,5.62);(18.12,5.62);(18.12,11.88);(18.12,11.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18,4)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<parallelogram p3= "(21.88,12)"
%	 p2= "(21.88,18.01)"
%	 p1= "(0,18.01)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(28.12,5.62);(28.12,5.62);(28.12,24.38);(28.12,24.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.12,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,16.25);(3.12,16.25);(3.12,26.25);(3.12,26.25)"
%	 />
%<parallelogram p3= "(31.88,24.5)"
%	 p2= "(31.88,30.5)"
%	 p1= "(0,30.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(28.12,30.62);(28.12,30.62);(28.12,38.12);(28.12,38.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.62,5.62);(15.62,5.62);(20.62,5.62);(20.62,5.62);(20.62,5.62);(18.12,0);
%	(18.12,0);(18.12,0);(15.62,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.62,5.62);(0.62,5.62);(5.62,5.62);(5.62,5.62);(5.62,5.62);(3.14,0);
%	(3.14,0);(3.14,0);(0.62,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,5.62);(25.62,5.62);(30.62,5.62);(30.62,5.62);(30.62,5.62);(28.14,0);
%	(28.14,0);(28.14,0);(25.62,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,28.75);(1.88,28.75);(4.38,28.75);(4.38,28.75);(4.38,28.75);(3.12,26.25);
%	(3.12,26.25);(3.12,26.25);(1.88,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,16.25);(1.88,16.25);(4.38,16.25);(4.38,16.25);(4.38,16.25);(3.12,13.75);
%	(3.12,13.75);(3.12,13.75);(1.88,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qhh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(31.88,38.12)
\rput(3.12,3.75){$\dh$}
\psline{->}(3.12,5.62)(3.12,13.75)
\psline{->}(18.12,5.62)(18.12,11.88)
\rput(18,4){$\bhh$}
\pspolygon[](0,18.01)(21.88,18.01)(21.88,12)(0,12)
\rput(13.12,15){$\ahh$}
\psline{->}(28.12,5.62)(28.12,24.38)
\rput(28.12,3.75){$\chh$}
\psline{->}(3.12,16.25)(3.12,26.25)
\pspolygon[](0,30.5)(31.88,30.5)(31.88,24.5)(0,24.5)
\psline{->}(28.12,30.62)(28.12,38.12)
\pspolygon(15.62,5.62)
(20.62,5.62)
(18.12,0)(15.62,5.62)
\pspolygon(0.62,5.62)
(5.62,5.62)
(3.14,0)(0.62,5.62)
\pspolygon(25.62,5.62)
(30.62,5.62)
(28.14,0)(25.62,5.62)
\pspolygon(1.88,28.75)
(4.38,28.75)
(3.12,26.25)(1.88,28.75)
\pspolygon(1.88,16.25)
(4.38,16.25)
(3.12,13.75)(1.88,16.25)
\rput(16.88,27.5){$\qhh$}
\end{pspicture}


==> PIC/lambda-u.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 11:50:47 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="21.88" y-min="4.38" y-max="30.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10);(3.12,10);(3.12,17.5);(3.12,17.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(18.12,10);(18.12,10);(18.12,15.62);(18.12,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.12,8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<parallelogram p3= "(21.88,15.75)"
%	 p2= "(21.88,21.76)"
%	 p1= "(0,21.76)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.88,18.76)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(18.12,21.88);(18.12,21.88);(18.12,30.62);(18.12,30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,20);(1.88,20);(4.38,20);(4.38,20);(4.38,20);(3.12,17.5);
%	(3.12,17.5);(3.12,17.5);(1.88,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.62,10);(0.62,10);(5.62,10);(5.62,10);(5.62,10);(3.12,4.38);
%	(3.12,4.38);(3.12,4.38);(0.62,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.62,10);(15.62,10);(20.62,10);(20.62,10);(20.62,10);(18.13,4.38);
%	(18.13,4.38);(18.13,4.38);(15.62,10)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(21.88,30.62)
\rput(3.12,8.12){$\dh$}
\psline{->}(3.12,10)(3.12,17.5)
\psline{->}(18.12,10)(18.12,15.62)
\rput(18.12,8.12){$\bhh$}
\pspolygon[](0,21.76)(21.88,21.76)(21.88,15.75)(0,15.75)
\rput(11.88,18.76){$\ahh$}
\psline{->}(18.12,21.88)(18.12,30.62)
\pspolygon(1.88,20)
(4.38,20)
(3.12,17.5)(1.88,20)
\pspolygon(0.62,10)
(5.62,10)
(3.12,4.38)(0.62,10)
\pspolygon(15.62,10)
(20.62,10)
(18.13,4.38)(15.62,10)
\end{pspicture}


==> PIC/moncat-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 11:27:47 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="65" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,34)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ih$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(65,53)
\rput(5,5){$\ah$}
\rput(15,34){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\rput(65,5){$\aah$}
\rput(35,5){$\ih$}
\end{pspicture}


==> PIC/moncat-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 11:43:05 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,34)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ih$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6,8);(6,8);(9,17);(9,17)"
%	 />
%<parallelogram p3= "(13,17)"
%	 p2= "(13,23)"
%	 p1= "(7,23)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11,23);(11,23);(13.75,31.25);(13.75,31.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,37);(17,37);(21,41);(21,41)"
%	 />
%<parallelogram p3= "(27,41)"
%	 p2= "(27,47)"
%	 p1= "(21,47)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(27,47);(27,47);(31,51);(31,51)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,44)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(36,8);(36,8);(39,17);(39,17)"
%	 />
%<parallelogram p3= "(43,17)"
%	 p2= "(43,23)"
%	 p1= "(37,23)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(41,23);(41,23);(44,32);(44,32)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22);(65,22)"
%	 />
%<parallelogram p3= "(68,22)"
%	 p2= "(68,28)"
%	 p1= "(62,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,28);(65,28);(65,42);(65,42)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53)
\rput(5,5){$\ah$}
\rput(15,34){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\rput(35,5){$\ih$}
\psline{->}(6,8)(9,17)
\pspolygon[](7,23)(13,23)(13,17)(7,17)
\psline{->}(11,23)(13.75,31.25)
\rput(10,20){$\af$}
\psline{->}(17,37)(21,41)
\pspolygon[](21,47)(27,47)(27,41)(21,41)
\psline{->}(27,47)(31,51)
\rput(24,44){$\ag$}
\psline{->}(36,8)(39,17)
\pspolygon[](37,23)(43,23)(43,17)(37,17)
\psline{->}(41,23)(44,32)
\rput(40,20){$\ak$}
\psline{->}(65,8)(65,22)
\pspolygon[](62,28)(68,28)(68,22)(62,22)
\psline{->}(65,28)(65,42)
\rput(65,25){$\ahh$}
\rput(65,5){$\aah$}
\end{pspicture}


==> PIC/moncat-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 15:16:39 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,34)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34,53)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6,8);(6,8);(9,17);(9,17)"
%	 />
%<parallelogram p3= "(13,17)"
%	 p2= "(13,23)"
%	 fill-style= "none"
%	 p1= "(7,23)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11,23);(11,23);(13.75,31.25);(13.75,31.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,37);(17,37);(21,41);(21,41)"
%	 />
%<parallelogram p3= "(27,41)"
%	 p2= "(27,47)"
%	 fill-style= "none"
%	 p1= "(21,47)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(27,47);(27,47);(31,51);(31,51)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(24,44)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(40.62,22.5);(40.62,22.5);(44,32);(44,32)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22);(65,22)"
%	 />
%<parallelogram p3= "(68,22)"
%	 p2= "(68,28)"
%	 fill-style= "none"
%	 p1= "(62,28)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,28);(65,28);(65,42);(65,42)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(36.88,22.5);(36.88,22.5);(43.75,22.5);(43.75,22.5);(43.75,22.5);(40,16.25);
%	(40,16.25);(40,16.25);(36.88,22.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53)
\rput(5,5){$\ah$}
\rput(15,34){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\psline{->}(6,8)(9,17)
\pspolygon[](7,23)(13,23)(13,17)(7,17)
\psline{->}(11,23)(13.75,31.25)
\rput(10,20){$\af$}
\psline{->}(17,37)(21,41)
\pspolygon[](21,47)(27,47)(27,41)(21,41)
\psline{->}(27,47)(31,51)
\rput(24,44){$\ag$}
\psline{->}(40.62,22.5)(44,32)
\rput(40,20){$\ak$}
\psline{->}(65,8)(65,22)
\pspolygon[](62,28)(68,28)(68,22)(62,22)
\psline{->}(65,28)(65,42)
\rput(65,25){$\ahh$}
\rput(65,5){$\aah$}
\pspolygon(36.88,22.5)
(43.75,22.5)
(40,16.25)(36.88,22.5)
\end{pspicture}


==> PIC/moncat-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 11:48:49 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6,8);(6,8);(9,17);(9,17)"
%	 />
%<parallelogram p3= "(13,17)"
%	 p2= "(13,23)"
%	 p1= "(7,23)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11,23);(11,23);(22.5,40.62);(22.5,40.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(27,41)"
%	 p2= "(27,47)"
%	 p1= "(21,47)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(27,47);(27,47);(31,51);(31,51)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,44)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(40.62,22.5);(40.62,22.5);(44,32);(44,32)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22);(65,22)"
%	 />
%<parallelogram p3= "(68,22)"
%	 p2= "(68,28)"
%	 p1= "(62,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,28);(65,28);(65,42);(65,42)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(36.88,22.5);(36.88,22.5);(43.75,22.5);(43.75,22.5);(43.75,22.5);(40,16.25);
%	(40,16.25);(40,16.25);(36.88,22.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53)
\rput(5,5){$\ah$}
\rput(14.38,33.75){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\psline{->}(6,8)(9,17)
\pspolygon[](7,23)(13,23)(13,17)(7,17)
\psline{->}(11,23)(22.5,40.62)
\rput(10,20){$\af$}
\pspolygon[](21,47)(27,47)(27,41)(21,41)
\psline{->}(27,47)(31,51)
\rput(24,44){$\ag$}
\psline{->}(40.62,22.5)(44,32)
\rput(40,20){$\ak$}
\psline{->}(65,8)(65,22)
\pspolygon[](62,28)(68,28)(68,22)(62,22)
\psline{->}(65,28)(65,42)
\rput(65,25){$\ahh$}
\rput(65,5){$\aah$}
\pspolygon(36.88,22.5)
(43.75,22.5)
(40,16.25)(36.88,22.5)
\end{pspicture}


==> PIC/moncat-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 23 16:50:08 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.62" x-max="28" y-min="5" y-max="53.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(0.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(4,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,7.5);(5,7.5);(5,21.88);(5,21.88)"
%	 />
%<parallelogram p3= "(8,22)"
%	 p2= "(8,28)"
%	 p1= "(2,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,28.12);(5,28.12);(5,36.88);(5,36.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(8,37)"
%	 p2= "(8,43)"
%	 p1= "(2,43)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,43.12);(5,43.12);(5,50);(5,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(15.62,18.12);(15.62,18.12);(15.62,50);(15.62,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,8);(25,8);(25,22);(25,22)"
%	 />
%<parallelogram p3= "(28,22)"
%	 p2= "(28,28)"
%	 p1= "(22,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,28);(25,28);(25,50);(25,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,18.12);(11.88,18.12);(18.75,18.12);(18.75,18.12);(18.75,18.12);(15,11.88);
%	(15,11.88);(15,11.88);(11.88,18.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28,53.12)
\rput(0.62,32.5){$\bh$}
\rput(4,53){$\ch$}
\rput(14.38,53.12){$\chh$}
\rput(25,53.12){$\dh$}
\psline{->}(5,7.5)(5,21.88)
\pspolygon[](2,28)(8,28)(8,22)(2,22)
\psline{->}(5,28.12)(5,36.88)
\rput(5,25){$\af$}
\pspolygon[](2,43)(8,43)(8,37)(2,37)
\psline{->}(5,43.12)(5,50)
\rput(5,40){$\ag$}
\psline{->}(15.62,18.12)(15.62,50)
\rput(15,15.62){$\ak$}
\psline{->}(25,8)(25,22)
\pspolygon[](22,28)(28,28)(28,22)(22,22)
\psline{->}(25,28)(25,50)
\rput(25,25){$\ahh$}
\rput(25,5){$\aah$}
\pspolygon(11.88,18.12)
(18.75,18.12)
(15,11.88)(11.88,18.12)
\rput(5,5){$\aah$}
\end{pspicture}


==> PIC/moncat-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 12:15:11 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="4.38" y-max="53.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40.62,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,7.5);(45,7.5);(45,15.62);(45,15.62)"
%	 />
%<parallelogram p3= "(48,15.75)"
%	 p2= "(48,21.75)"
%	 p1= "(42,21.75)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,21.88);(45,21.88);(45,36.88);(45,36.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(48,37)"
%	 p2= "(48,43)"
%	 p1= "(42,43)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,43.12);(45,43.12);(45,50);(45,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55.62,48.75);(55.62,48.75);(55.62,50);(55.62,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,8.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,36.88);(65,36.88)"
%	 />
%<parallelogram p3= "(68,37)"
%	 p2= "(68,43)"
%	 p1= "(62,43)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,43.12);(65,43.12);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(26.88,10.62);(26.88,10.62);(33.75,10.62);(33.75,10.62);(33.75,10.62);(30,4.38);
%	(30,4.38);(30,4.38);(26.88,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,10.62);(30,10.62);(30,22.5);(34.38,26.25);(38.75,30);(41.88,30);
%	(45,31.25);(48.12,32.5);(50,33.75);(52.5,37.5);(55,41.25);(55.62,49.38);
%	(55.62,49.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53.12)
\rput(5,5){$\ah$}
\rput(40.62,25){$\bh$}
\rput(44,53){$\ch$}
\rput(54.38,53.12){$\chh$}
\rput(65,53.12){$\dh$}
\psline{->}(45,7.5)(45,15.62)
\pspolygon[](42,21.75)(48,21.75)(48,15.75)(42,15.75)
\psline{->}(45,21.88)(45,36.88)
\rput(45,18.75){$\af$}
\pspolygon[](42,43)(48,43)(48,37)(42,37)
\psline{->}(45,43.12)(45,50)
\rput(45,40){$\ag$}
\psline{->}(55.62,48.75)(55.62,50)
\rput(30,8.12){$\ak$}
\psline{->}(65,8)(65,36.88)
\pspolygon[](62,43)(68,43)(68,37)(62,37)
\psline{->}(65,43.12)(65,50)
\rput(65,40){$\ahh$}
\rput(65,5){$\aah$}
\pspolygon(26.88,10.62)
(33.75,10.62)
(30,4.38)(26.88,10.62)
\rput(45,5){$\aah$}
\pscustom[]{\psbezier(30,10.62)(30,10.62)(30,22.5)(34.38,26.25)
\psbezier(38.75,30)(41.88,30)(45,31.25)
\psbezier(48.12,32.5)(50,33.75)(52.5,37.5)
\psbezier(55,41.25)(55.62,49.38)(55.62,49.38)
}
\end{pspicture}


==> PIC/moncat-7.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 12:29:48 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,7.5);(45,7.5);(45,22.5);(45,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,37.5);(45,37.5);(45,50);(45,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55.62,37.5);(55.62,37.5);(55.62,50);(55.62,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22.5);(65,22.5)"
%	 />
%<parallelogram p3= "(68,22.5)"
%	 p2= "(68,37.5)"
%	 p1= "(42,37.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,37.5);(65,37.5);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\formula$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eql$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53.12)
\rput(5,5){$\ah$}
\rput(44,53){$\ch$}
\rput(54.38,53.12){$\chh$}
\rput(65,53.12){$\dh$}
\psline{->}(45,7.5)(45,22.5)
\psline{->}(45,37.5)(45,50)
\psline{->}(55.62,37.5)(55.62,50)
\psline{->}(65,8)(65,22.5)
\pspolygon[](42,37.5)(68,37.5)(68,22.5)(42,22.5)
\psline{->}(65,37.5)(65,50)
\rput(55,25.62){$\ahh$}
\rput(65,5){$\aah$}
\rput(45,5){$\aah$}
\rput(55,33.75){$\formula$}
\rput(55,30){$\eql$}
\end{pspicture}


==> PIC/moncat-8.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 13:17:16 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68.25" y-min="-1" y-max="55" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.12,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(50,12);(50,12);(45,22.5);(45,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,37.5);(45,37.5);(45,50);(45,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55.62,37.5);(55.62,37.5);(55.62,50);(55.62,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(60,12);(60,12);(65,22.5);(65,22.5)"
%	 />
%<parallelogram p3= "(68,22.5)"
%	 p2= "(68,37.5)"
%	 p1= "(42,37.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,37.5);(65,37.5);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,-1)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\formula$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eql$
%</text>
%<multicurve fill-style= "none"
%	 points= "(47,12);(47,12);(63.25,12);(63.25,12);(63.25,12);(58.25,7);
%	(58.25,7);(58.25,7);(52,7);(52,7);(52,7);(47,12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55,2);(55,2);(55,7);(55,7)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(62,50);(62,50);(68.25,50);(68.25,50);(68.25,50);(65.12,55);
%	(65.12,55);(65.12,55);(65.12,55);(65.12,55);(65.12,55);(62,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,52)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65.62,16.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,16.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68.25,55)
\rput(5,5){$\ah$}
\rput(44,53){$\ch$}
\rput(54.38,53.12){$\chh$}
\rput(68.12,43.12){$\dh$}
\psline{->}(50,12)(45,22.5)
\psline{->}(45,37.5)(45,50)
\psline{->}(55.62,37.5)(55.62,50)
\psline{->}(60,12)(65,22.5)
\pspolygon[](42,37.5)(68,37.5)(68,22.5)(42,22.5)
\psline{->}(65,37.5)(65,50)
\rput(55,25.62){$\ahh$}
\rput(55,-1){$\aah$}
\rput(55,33.75){$\formula$}
\rput(55,30){$\eql$}
\pspolygon(47,12)
(63.25,12)
(58.25,7)
(52,7)(47,12)
\psline{->}(55,2)(55,7)
\rput(55,9.38){$\diagonal$}
\pscustom[]{\psline(62,50)(68.25,50)
\psline(68.25,50)(65.12,55)
\psbezier(65.12,55)(65.12,55)(65.12,55)
\psline(65.12,55)(62,50)
\closepath}
\rput(65,52){$\delete$}
\rput(65.62,16.88){$\aah$}
\rput(44.38,16.88){$\aah$}
\end{pspicture}


==> PIC/moncat-9.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 25 11:05:37 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="28.25" y-min="-1" y-max="65" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.12,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(10,12);(10,12);(5,22.5);(5,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,37.5);(5,37.5);(5,50);(5,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(15.62,37.5);(15.62,37.5);(15.62,50);(15.62,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(20,12);(20,12);(25,22.5);(25,22.5)"
%	 />
%<parallelogram p3= "(28,22.5)"
%	 p2= "(28,37.5)"
%	 p1= "(2,37.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,37.5);(25,37.5);(25,50);(25,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,-1)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\formula$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eql$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7,12);(7,12);(23.25,12);(23.25,12);(23.25,12);(18.25,7);
%	(18.25,7);(18.25,7);(12,7);(12,7);(12,7);(7,12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(15,2);(15,2);(15,7);(15,7)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(22,50);(22,50);(28.25,50);(28.25,50);(28.25,50);(25.12,55);
%	(25.12,55);(25.12,55);(25.12,55);(25.12,55);(25.12,55);(22,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,52)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\delete$
%</text>
%<multicurve fill-style= "none"
%	 points= "(18.25,50);(18.25,50);(2,50);(2,50);(2,50);(7,55);
%	(7,55);(7,55);(13.25,55);(13.25,55);(13.25,55);(18.25,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(10,55);(10,55);(10,62);(10,62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,52.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\codiagonal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.62,16.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(4.38,16.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28.25,65)
\rput(10,65){$\ch$}
\rput(28.12,43.12){$\dh$}
\psline{->}(10,12)(5,22.5)
\psline{->}(5,37.5)(5,50)
\psline{->}(15.62,37.5)(15.62,50)
\psline{->}(20,12)(25,22.5)
\pspolygon[](2,37.5)(28,37.5)(28,22.5)(2,22.5)
\psline{->}(25,37.5)(25,50)
\rput(15,25.62){$\ahh$}
\rput(15,-1){$\aah$}
\rput(15,33.75){$\formula$}
\rput(15,30){$\eql$}
\pspolygon(7,12)
(23.25,12)
(18.25,7)
(12,7)(7,12)
\psline{->}(15,2)(15,7)
\rput(15,9.38){$\diagonal$}
\pscustom[]{\psline(22,50)(28.25,50)
\psline(28.25,50)(25.12,55)
\psbezier(25.12,55)(25.12,55)(25.12,55)
\psline(25.12,55)(22,50)
\closepath}
\rput(25,52){$\delete$}
\pspolygon(18.25,50)
(2,50)
(7,55)
(13.25,55)(18.25,50)
\psline{->}(10,55)(10,62)
\rput(10,52.5){$\codiagonal$}
\rput(25.62,16.88){$\aah$}
\rput(4.38,16.88){$\aah$}
\rput(1.88,43.12){$\ch$}
\rput(18.75,43.12){$\ch$}
\end{pspicture}


==> PIC/norm.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 23 14:40:22 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="6.25" y-min="8.12" y-max="27.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,11.88);(3.12,11.88);(3.12,24.38);(3.12,24.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,10.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.25,24.38);(6.25,24.38);(0,24.38);(0,24.38);(0,24.38);(3.12,27.5);
%	(3.12,27.5);(3.12,27.5);(3.12,27.5);(3.12,27.5);(3.12,27.5);(6.25,24.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,11.88);(6.25,11.88);(0,11.88);(0,11.88);(0,11.88);(3.12,8.12);
%	(3.12,8.12);(3.12,8.12);(3.12,8.12);(3.12,8.12);(3.12,8.12);(6.25,11.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(6.25,27.5)
\psline{->}(3.12,11.88)(3.12,24.38)
\rput(3.12,10.62){$\one$}
\pscustom[]{\psline(6.25,24.38)(0,24.38)
\psline(0,24.38)(3.12,27.5)
\psbezier(3.12,27.5)(3.12,27.5)(3.12,27.5)
\psline(3.12,27.5)(6.25,24.38)
\closepath}
\pscustom[]{\psline(6.25,11.88)(0,11.88)
\psline(0,11.88)(3.12,8.12)
\psbezier(3.12,8.12)(3.12,8.12)(3.12,8.12)
\psline(3.12,8.12)(6.25,11.88)
\closepath}
\end{pspicture}


==> PIC/normform-cx-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 20 07:04:52 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="32.5" y-min="-18.75" y-max="33.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20.62,14.38)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(18.12,-6.24);(18.12,-6.24);(18.12,-2.5);(18.12,-2.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(19.37,16.26);(19.37,16.26);(23.75,20.62);(23.75,20.62)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,-18.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(14.38,1.26);(14.38,1.26);(22.5,-6.86);(22.5,-6.86);(22.5,-6.86);(22.5,-6.86);
%	(22.5,-6.86);(22.5,-6.86);(22.5,3.76);(22.5,3.76);(22.5,3.76);(14.38,11.88);
%	(14.38,11.88);(14.38,11.88);(14.38,1.26);(14.38,1.26);(14.38,1.26);(14.38,1.26);
%	(14.38,1.26);(14.38,1.26);(14.38,8.76);(14.38,8.76)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(14.38,16.25);(14.38,16.25);(23.12,16.25);(23.12,16.25);(23.12,16.25);(23.12,7.5);
%	(23.12,7.5);(23.12,7.5);(22.5,8.1);(22.5,8.1);(22.5,8.1);(14.38,16.25);
%	(14.38,16.25)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(18.75,7.5);(18.75,7.5);(18.75,11.88);(18.75,11.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(5.62,-15);(5.62,-15);(5.62,-5.62);(5.62,-5.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(16.25,-14.86);(16.25,-14.86);(16.25,-10.63);(16.25,-10.63)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,-18.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,-6.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve points= "(1.88,-1.87);(1.88,-1.87);(10.62,-10.63);(10.62,-10.63);(10.62,-10.63);(22.5,-10.63);
%	(22.5,-10.63);(22.5,-10.63);(13.75,-1.87);(13.75,-1.87);(13.75,-1.87);(13.75,-1.88);
%	(13.75,-1.88);(13.75,-1.88);(1.88,-1.88);(1.88,-1.88);(1.88,-1.88);(1.88,-1.87);
%	(1.88,-1.87);(1.88,-1.87);(1.88,-1.87);(1.88,-1.87)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,3.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\thh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.62,-18.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Fhh$
%</text>
%<ellipse p3= "(29.69,19.69)"
%	 p2= "(29.69,26.56)"
%	 p1= "(22.81,26.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "none"
%	 angle-start= "0"
%	 />
%<multicurve left-arrow= "head"
%	 points= "(28.75,20.62);(28.75,20.62);(32.5,16.88);(32.5,16.88);(32.5,16.88);(32.5,-14.38);
%	(32.5,-14.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,23.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\order$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(26.25,26.88);(26.25,26.88);(26.25,31.25);(26.25,31.25)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,33.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Tval$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(32.5,33.75)
\rput(20.62,14.38){$\ahh$}
\psline{->}(18.12,-6.24)(18.12,-2.5)
\psline{->}(19.37,16.26)(23.75,20.62)
\rput(32.5,-18.75){$\Lhh$}
\pscustom[]{\psline(14.38,1.26)(22.5,-6.86)
\psbezier(22.5,-6.86)(22.5,-6.86)(22.5,-6.86)
\psline(22.5,-6.86)(22.5,3.76)
\psline(22.5,3.76)(14.38,11.88)
\psline(14.38,11.88)(14.38,1.26)
\psbezier(14.38,1.26)(14.38,1.26)(14.38,1.26)
\psline(14.38,1.26)(14.38,8.76)
}
\psline(14.38,16.25)
(23.12,16.25)
(23.12,7.5)
(22.5,8.1)(14.38,16.25)
\psline{->}(18.75,7.5)(18.75,11.88)
\psline{->}(5.62,-15)(5.62,-5.62)
\psline{->}(16.25,-14.86)(16.25,-10.63)
\rput(16.25,-18.75){$\bhh$}
\rput(13.12,-6.25){$\shh$}
\pscustom[]{\psline(1.88,-1.87)(10.62,-10.63)
\psline(10.62,-10.63)(22.5,-10.63)
\psline(22.5,-10.63)(13.75,-1.87)
\psline(13.75,-1.87)(13.75,-1.88)
\psline(13.75,-1.88)(1.88,-1.88)
\psline(1.88,-1.88)(1.88,-1.87)
\psbezier(1.88,-1.87)(1.88,-1.87)(1.88,-1.87)
}
\rput(18.75,3.12){$\thh$}
\rput(5.62,-18.75){$\Fhh$}
\rput{0}(26.25,23.12){\psellipse[](0,0)(3.44,-3.43)}
\psline{<-}(28.75,20.62)
(32.5,16.88)(32.5,-14.38)
\rput(26.25,23.12){$\order$}
\psline{->}(26.25,26.88)(26.25,31.25)
\rput(26.25,33.75){$\Tval$}
\end{pspicture}


==> PIC/normform-cx-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 20 07:05:18 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="38.12" y-min="-18.75" y-max="33.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,5.62)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(18.12,-6.24);(18.12,-6.24);(18.12,-2.5);(18.12,-2.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(33.75,-18.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(14.38,1.26);(14.38,1.26);(22.5,-6.86);(22.5,-6.86);(22.5,-6.86);(22.5,-6.86);
%	(22.5,-6.86);(22.5,-6.86);(22.5,3.76);(22.5,3.76);(22.5,3.76);(14.38,11.88);
%	(14.38,11.88);(14.38,11.88);(14.38,1.26);(14.38,1.26);(14.38,1.26);(14.38,1.26);
%	(14.38,1.26);(14.38,1.26);(14.38,8.76);(14.38,8.76)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(38.12,3.12);(38.12,3.12);(29.37,3.12);(29.37,3.12);(29.37,3.12);(29.37,11.87);
%	(29.37,11.87);(29.37,11.87);(30,11.27);(30,11.27);(30,11.27);(38.12,3.12);
%	(38.12,3.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(33.75,-15);(33.75,-15);(33.75,3.12);(33.75,3.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(5.62,-15);(5.62,-15);(5.62,-5.62);(5.62,-5.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(16.25,-14.86);(16.25,-14.86);(16.25,-10.63);(16.25,-10.63)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,-18.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(12.5,-6.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve points= "(1.88,-1.87);(1.88,-1.87);(10.62,-10.63);(10.62,-10.63);(10.62,-10.63);(22.5,-10.63);
%	(22.5,-10.63);(22.5,-10.63);(13.75,-1.87);(13.75,-1.87);(13.75,-1.87);(13.75,-1.88);
%	(13.75,-1.88);(13.75,-1.88);(1.88,-1.88);(1.88,-1.88);(1.88,-1.88);(1.88,-1.87);
%	(1.88,-1.87);(1.88,-1.87);(1.88,-1.87);(1.88,-1.87)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,3.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\thh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.62,-18.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Fhh$
%</text>
%<ellipse p3= "(29.69,19.69)"
%	 p2= "(29.69,26.56)"
%	 p1= "(22.81,26.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "none"
%	 angle-start= "0"
%	 />
%<multicurve left-arrow= "head"
%	 points= "(23.75,20.62);(23.75,20.62);(18.75,15.62);(18.75,15.62);(18.75,15.62);(18.75,7.5);
%	(18.75,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,23.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\order$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(26.25,26.88);(26.25,26.88);(26.25,31.25);(26.25,31.25)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,33.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Tval$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20.62,13.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve left-arrow= "head"
%	 points= "(28.75,20.62);(28.75,20.62);(33.75,15.62);(33.75,15.62);(33.75,15.62);(33.75,7.5);
%	(33.75,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.88,11.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Fhh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(38.12,33.75)
\rput(32.5,5.62){$\ahh$}
\psline{->}(18.12,-6.24)(18.12,-2.5)
\rput(33.75,-18.75){$\Lhh$}
\pscustom[]{\psline(14.38,1.26)(22.5,-6.86)
\psbezier(22.5,-6.86)(22.5,-6.86)(22.5,-6.86)
\psline(22.5,-6.86)(22.5,3.76)
\psline(22.5,3.76)(14.38,11.88)
\psline(14.38,11.88)(14.38,1.26)
\psbezier(14.38,1.26)(14.38,1.26)(14.38,1.26)
\psline(14.38,1.26)(14.38,8.76)
}
\psline(38.12,3.12)
(29.37,3.12)
(29.37,11.87)
(30,11.27)(38.12,3.12)
\psline{->}(33.75,-15)(33.75,3.12)
\psline{->}(5.62,-15)(5.62,-5.62)
\psline{->}(16.25,-14.86)(16.25,-10.63)
\rput(16.25,-18.75){$\bhh$}
\rput(12.5,-6.25){$\shh$}
\pscustom[]{\psline(1.88,-1.87)(10.62,-10.63)
\psline(10.62,-10.63)(22.5,-10.63)
\psline(22.5,-10.63)(13.75,-1.87)
\psline(13.75,-1.87)(13.75,-1.88)
\psline(13.75,-1.88)(1.88,-1.88)
\psline(1.88,-1.88)(1.88,-1.87)
\psbezier(1.88,-1.87)(1.88,-1.87)(1.88,-1.87)
}
\rput(18.75,3.12){$\thh$}
\rput(5.62,-18.75){$\Fhh$}
\rput{0}(26.25,23.12){\psellipse[](0,0)(3.44,-3.43)}
\psline{<-}(23.75,20.62)
(18.75,15.62)(18.75,7.5)
\rput(26.25,23.12){$\order$}
\psline{->}(26.25,26.88)(26.25,31.25)
\rput(26.25,33.75){$\Tval$}
\rput(20.62,13.75){}
\psline{<-}(28.75,20.62)
(33.75,15.62)(33.75,7.5)
\rput(36.88,11.88){$\Fhh$}
\end{pspicture}


==> PIC/poly-diags.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 17:06:04 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="68" y-min="-9" y-max="45.07" auto-bounding="true">
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 anchor-point= "(40.75,-6)"
%	 fill-style= "none"
%	 arrow-tbar-width-linewidth-scale= "2"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(19,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\leftcat$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(49,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\rightcat$
%</text>
%<multicurve right-arrow= "head"
%	 left-arrow= "t-bar-flushed"
%	 fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(28.12,22.5);(28.12,22.5)"
%	 />
%<parallelogram p3= "(57.59,26.58)"
%	 p2= "(57.59,23.16)"
%	 p1= "(44.79,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.19,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle h$
%</text>
%<parallelogram p3= "(63.99,12.33)"
%	 p2= "(63.99,8.91)"
%	 p1= "(54.39,8.91)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(63.99,10.62)"
%	 p2= "(63.99,10.62)"
%	 p1= "(63.99,10.62)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(62.39,5.49);(62.39,5.49);(62.39,8.91);(62.39,8.91)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(56,-9);(56,-9);(55.99,8.91);(55.99,8.91)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(55.99,12.33);(55.99,12.33);(55.99,23.16);(55.99,23.16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(59.19,10.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram p3= "(63.99,26.58)"
%	 p2= "(63.99,23.16)"
%	 p1= "(59.19,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.59,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(59,-9);(59,-9);(59,9);(59,9)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(62.79,18.6);(62.79,18.6);(62.79,23.16);(62.79,23.16)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(47.99,26.58);(47.99,26.58);(48,36);(48,36)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(61.59,26.58);(61.59,26.58);(61.59,29.43);(61.59,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(54.39,26.58);(54.39,26.58);(54.38,35.93);(54.38,35.93)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(59.99,29.43);(59.99,29.43);(61.59,31.71);(61.59,31.71);(61.59,31.71);(63.19,29.43);
%	(63.19,29.43);(63.19,29.43);(59.99,29.43);(59.99,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(46.44,15.75);(46.44,15.75);(46.44,22.88);(46.44,22.88)"
%	 />
%<parallelogram p3= "(15.59,26.58)"
%	 p2= "(15.59,23.16)"
%	 p1= "(2.79,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.19,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle h$
%</text>
%<parallelogram p3= "(21.99,12.33)"
%	 p2= "(21.99,8.91)"
%	 p1= "(12.39,8.91)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(21.99,10.62)"
%	 p2= "(21.99,10.62)"
%	 p1= "(21.99,10.62)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(14,-9);(14,-9);(13.99,8.91);(13.99,8.91)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(13.99,12.33);(13.99,12.33);(13.99,23.16);(13.99,23.16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.19,10.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram p3= "(21.99,26.58)"
%	 p2= "(21.99,23.16)"
%	 p1= "(17.19,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(19.59,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(17,-9);(17,-9);(17,9);(17,9)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(6,26.56);(6,26.56);(6,36);(6,36)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(19.59,26.58);(19.59,26.58);(19.59,29.43);(19.59,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(12.5,26.57);(12.5,26.57);(12.5,36.02);(12.5,36.02)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(17.99,29.43);(17.99,29.43);(19.59,31.71);(19.59,31.71);(19.59,31.71);(21.19,29.43);
%	(21.19,29.43);(21.19,29.43);(17.99,29.43);(17.99,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(4,2);(4,2);(4,23);(4,23)"
%	 />
%<parallelogram right-arrow= "head"
%	 p3= "(26,-2)"
%	 p2= "(26,33)"
%	 p1= "(0,33)"
%	 fill-style= "none"
%	 />
%<pscurve stroke-width= "0.12"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(20,9);(20,9);(19,6);(9,7);(7,6);(6.25,4.38);
%	(6,2);(6,2);(6,2);(6.25,1.88)"
%	 />
%<pscurve stroke-width= "0.15"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(8,2);(8,2);(8.75,5);(10.71,5.39);(21,3);(23.75,6.88);
%	(21.88,15.62);(21.25,18.12);(21,20);(21,23);(21,23)"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(6,-1);(6,-1);(6,-9);(6,-9)"
%	 />
%<pscurve right-arrow= "head"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(19,42);(19,42);(33,45);(49,42);(53,40)"
%	 />
%<pscurve right-arrow= "head"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(48.99,38.22);(48.99,38.22);(34.92,35.59);(19,39);(15.05,41.1)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(48.97,15.86);(48.97,15.86);(46.47,13.36);(46.47,13.36);(46.47,13.36);(43.97,15.86);
%	(43.97,15.86)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(65.36,18.54);(65.36,18.54);(62.86,16.04);(62.86,16.04);(62.86,16.04);(60.36,18.54);
%	(60.36,18.54)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(64.91,5.54);(64.91,5.54);(62.41,3.04);(62.41,3.04);(62.41,3.04);(59.91,5.54);
%	(59.91,5.54)"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5.67,-6.39)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\scriptstyle X$
%</text>
%<multicurve right-arrow= "head"
%	 stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(2.05,1.98);(2.05,1.98);(10.05,1.98);(10.05,1.98);(10.05,1.98);(8.05,-1.02);
%	(8.05,-1.02);(8.05,-1.02);(4.05,-1.02);(4.05,-1.02);(4.05,-1.02);(2.05,1.98)"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.03,0.39)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle \Delta$
%</text>
%<parallelogram right-arrow= "head"
%	 p3= "(68,-2)"
%	 p2= "(68,33)"
%	 p1= "(42,33)"
%	 fill-style= "none"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(34.46,24.09)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle \kappa x.$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,45.07)
\rput(40.75,-6){}
\rput[r](19,40){$\leftcat$}
\rput[l](49,40){$\rightcat$}
\psline{|*->}(40,22.5)(28.12,22.5)
\pspolygon[linewidth=0.12](44.79,23.16)(57.59,23.16)(57.59,26.58)(44.79,26.58)
\rput(51.19,24.87){$\scriptstyle h$}
\pspolygon[linewidth=0.12](54.39,8.91)(63.99,8.91)(63.99,12.33)(54.39,12.33)
\pspolygon[linewidth=0.12](63.99,10.62)(63.99,10.62)(63.99,10.62)(63.99,10.62)
\psline[linewidth=0.12](62.39,5.49)(62.39,8.91)
\psline[linewidth=0.12](56,-9)(55.99,8.91)
\psline[linewidth=0.12](55.99,12.33)(55.99,23.16)
\rput(59.19,10.62){$\scriptstyle g$}
\pspolygon[linewidth=0.12](59.19,23.16)(63.99,23.16)(63.99,26.58)(59.19,26.58)
\rput(61.59,24.87){$\scriptstyle f$}
\psline[linewidth=0.12](59,-9)(59,9)
\psline[linewidth=0.12](62.79,18.6)(62.79,23.16)
\psline[linewidth=0.12](47.99,26.58)(48,36)
\psline[linewidth=0.12](61.59,26.58)(61.59,29.43)
\psline[linewidth=0.12](54.39,26.58)(54.38,35.93)
\psline[linewidth=0.12](59.99,29.43)
(61.59,31.71)
(63.19,29.43)(59.99,29.43)
\psline[linewidth=0.12](46.44,15.75)(46.44,22.88)
\pspolygon[linewidth=0.12](2.79,23.16)(15.59,23.16)(15.59,26.58)(2.79,26.58)
\rput(9.19,24.87){$\scriptstyle h$}
\pspolygon[linewidth=0.12](12.39,8.91)(21.99,8.91)(21.99,12.33)(12.39,12.33)
\pspolygon[linewidth=0.12](21.99,10.62)(21.99,10.62)(21.99,10.62)(21.99,10.62)
\psline[linewidth=0.12](14,-9)(13.99,8.91)
\psline[linewidth=0.12](13.99,12.33)(13.99,23.16)
\rput(17.19,10.62){$\scriptstyle g$}
\pspolygon[linewidth=0.12](17.19,23.16)(21.99,23.16)(21.99,26.58)(17.19,26.58)
\rput(19.59,24.87){$\scriptstyle f$}
\psline[linewidth=0.12](17,-9)(17,9)
\psline[linewidth=0.12](6,26.56)(6,36)
\psline[linewidth=0.12](19.59,26.58)(19.59,29.43)
\psline[linewidth=0.12](12.5,26.57)(12.5,36.02)
\psline[linewidth=0.12](17.99,29.43)
(19.59,31.71)
(21.19,29.43)(17.99,29.43)
\psline[linewidth=0.12](4,2)(4,23)
\pspolygon[](0,33)(26,33)(26,-2)(0,-2)
\psecurve[linewidth=0.12,curvature=1.0 0.1 0.0](20,9)(20,9)(19,6)(9,7)(7,6)(6.25,4.38)(6,2)(6,2)(6,2)(6.25,1.88)
\psecurve[linewidth=0.15,curvature=1.0 0.1 0.0](8,2)(8,2)(8.75,5)(10.71,5.39)(21,3)(23.75,6.88)(21.88,15.62)(21.25,18.12)(21,20)(21,23)(21,23)
\psline[linewidth=0.15](6,-1)(6,-9)
\psecurve{->}(19,42)(19,42)(33,45)(49,42)(53,40)
\psecurve{->}(48.99,38.22)(48.99,38.22)(34.92,35.59)(19,39)(15.05,41.1)
\psline[linewidth=0.05,fillstyle=solid](48.97,15.86)
(46.47,13.36)(43.97,15.86)
\psline[linewidth=0.05,fillstyle=solid](65.36,18.54)
(62.86,16.04)(60.36,18.54)
\psline[linewidth=0.05,fillstyle=solid](64.91,5.54)
(62.41,3.04)(59.91,5.54)
\rput[r](5.67,-6.39){$\scriptstyle X$}
\pspolygon[linewidth=0.15](2.05,1.98)
(10.05,1.98)
(8.05,-1.02)
(4.05,-1.02)(2.05,1.98)
\rput(6.03,0.39){$\scriptstyle \Delta$}
\pspolygon[](42,33)(68,33)(68,-2)(42,-2)
\rput(34.46,24.09){$\scriptstyle \kappa x.$}
\end{pspicture}


==> PIC/poly.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 16:46:34 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="52.5" y-min="0" y-max="23.12" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 left-arrow= "reverse-head"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 points= "(5.12,13);(5.12,13);(24.12,22);(24.12,22)"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 points= "(5.12,11);(5.12,11);(25.12,2);(25.12,2)"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-tbar-width-minimum= "0.15"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(28.12,20);(28.12,20);(28.12,3.12);(28.12,3.12)"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 anchor-point= "(36.12,0)"
%	 fill-style= "none"
%	 arrow-tbar-width-linewidth-scale= "2"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve right-arrow= "head"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 points= "(51.25,20);(51.25,20);(51.25,3.12);(51.25,3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.62,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Polycat$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Target$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\target$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,11.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Category$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(13.75,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Functor$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(29.38,11.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Indfunctor$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(13.75,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Unit$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(52.5,23.12)
\psline[tbarsize=0.15 5]{>->}(5.12,13)(24.12,22)
\psline[tbarsize=0.15 5]{->}(5.12,11)(25.12,2)
\psline[linestyle=dashed,dash=1 1,tbarsize=0.15 5]{->}(28.12,20)(28.12,3.12)
\rput(36.12,0){}
\psline[tbarsize=0.15 5]{|*->}(51.25,20)(51.25,3.12)
\rput[l](25.62,23.12){$\Polycat$}
\rput[l](26.25,0.62){$\Target$}
\rput(52.5,23.12){$\variable$}
\rput(52.5,0.62){$\target$}
\rput[r](3.75,11.88){$\Category$}
\rput[t](13.75,5){$\Functor$}
\rput[l](29.38,11.88){$\Indfunctor$}
\rput[b](13.75,18.75){$\Unit$}
\end{pspicture}


==> PIC/program.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 17:28:12 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.13" x-max="10" y-min="-6" y-max="7" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,0);(5,0);(5,5);(5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-2)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0.13,0);(0.13,0);(10,0);(10,0);(10,0);(5,-6);
%	(5,-6);(5,-6);(0.13,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,7)
\rput(5,7){$\chh$}
\psline{->}(5,0)(5,5)
\rput(5,-2){$\ak$}
\pspolygon(0.13,0)
(10,0)
(5,-6)(0.13,0)
\end{pspicture}


==> PIC/resource-photos.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Aug 22 18:20:55 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8.75" x-max="42.5" y-min="3.75" y-max="97.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Resource
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Residue
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\utility
%</text>
%<text text-vert-align= "center-v"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.5"
%	 anchor-point= "(15,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\investment
%</text>
%<multicurve right-arrow= "double-head"
%	 fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(30,72.5);(30,72.5);(30,25);(30,25)"
%	 />
%<multicurve stroke-dotsep= "5"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "1.3"
%	 stroke-style= "dotted"
%	 points= "(20,25);(20,25);(20,72.5);(20,72.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\coal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ashes
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\burn
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\store
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(42.5,97.5)
\rput(25,85){\Resource}
\rput(25,15){\Residue}
\rput[l](35,50){\utility}
\rput[r](15,50){\investment}
\psline[linewidth=0.6]{->>}(30,72.5)(30,25)
\psline[linewidth=1.3,linestyle=dotted,dotsep=5]{->}(20,25)(20,72.5)
\rput(25,97.5){\coal}
\rput(25,3.75){\ashes}
\rput(42.5,36.25){\burn}
\rput(8.75,65){\store}
\end{pspicture}


==> PIC/resource.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Aug 22 17:36:54 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15" x-max="35" y-min="5" y-max="75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Resource
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Residue
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\utility
%</text>
%<text text-vert-align= "center-v"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.5"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\investment
%</text>
%<multicurve right-arrow= "double-head"
%	 fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(30,62.5);(30,62.5);(30,15);(30,15)"
%	 />
%<multicurve stroke-dotsep= "5"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "1.3"
%	 stroke-style= "dotted"
%	 points= "(20,15);(20,15);(20,62.5);(20,62.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,75)
\rput(25,75){\Resource}
\rput(25,5){\Residue}
\rput[l](35,40){\utility}
\rput[r](15,40){\investment}
\psline[linewidth=0.6]{->>}(30,62.5)(30,15)
\psline[linewidth=1.3,linestyle=dotted,dotsep=5]{->}(20,15)(20,62.5)
\end{pspicture}


==> PIC/semigroup-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 24 07:18:52 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1" x-max="65" y-min="-0" y-max="26" auto-bounding="true">
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(15,16);(15,16);(15,-0);(15,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(17,16);(17,16);(5,16);(5,16);(5,16);(8,20);
%	(8,20);(8,20);(14,20);(14,20);(14,20);(17,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(11,20);(11,20);(11,26);(11,26)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(7,16);(7,16);(7,10);(7,10)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(11,6);(11,6);(11,-0);(11,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(13,6);(13,6);(1,6);(1,6);(1,6);(4,10);
%	(4,10);(4,10);(10,10);(10,10);(10,10);(13,6)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(3,6);(3,6);(3,-0);(3,-0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22,13)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(31,16);(31,16);(31,-0);(31,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(41,16);(41,16);(29,16);(29,16);(29,16);(32,20);
%	(32,20);(32,20);(38,20);(38,20);(38,20);(41,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(35,20);(35,20);(35,26);(35,26)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(39,16);(39,16);(39,10);(39,10)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(43,6);(43,6);(43,-0);(43,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(45,6);(45,6);(33,6);(33,6);(33,6);(36,10);
%	(36,10);(36,10);(42,10);(42,10);(42,10);(45,6)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(35,6);(35,6);(35,-0);(35,-0)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(63,16);(63,16);(63,-0);(63,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(65,16);(65,16);(53,16);(53,16);(53,16);(56,20);
%	(56,20);(56,20);(62,20);(62,20);(62,20);(65,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(59,20);(59,20);(59,26);(59,26)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(55,16);(55,16);(55,-0);(55,-0)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(59,16);(59,16);(59,-0);(59,-0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(49,13)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(39,8)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,18)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7,8)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11,18)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59,18)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comontwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(65,26)
\psline[linewidth=0.22](15,16)(15,-0)
\pspolygon[linewidth=0.22](17,16)
(5,16)
(8,20)
(14,20)(17,16)
\psline[linewidth=0.22](11,20)(11,26)
\psline[linewidth=0.22](7,16)(7,10)
\psline[linewidth=0.22](11,6)(11,-0)
\pspolygon[linewidth=0.22](13,6)
(1,6)
(4,10)
(10,10)(13,6)
\psline[linewidth=0.22](3,6)(3,-0)
\rput(22,13){$=$}
\psline[linewidth=0.22](31,16)(31,-0)
\pspolygon[linewidth=0.22](41,16)
(29,16)
(32,20)
(38,20)(41,16)
\psline[linewidth=0.22](35,20)(35,26)
\psline[linewidth=0.22](39,16)(39,10)
\psline[linewidth=0.22](43,6)(43,-0)
\pspolygon[linewidth=0.22](45,6)
(33,6)
(36,10)
(42,10)(45,6)
\psline[linewidth=0.22](35,6)(35,-0)
\psline[linewidth=0.22](63,16)(63,-0)
\pspolygon[linewidth=0.22](65,16)
(53,16)
(56,20)
(62,20)(65,16)
\psline[linewidth=0.22](59,20)(59,26)
\psline[linewidth=0.22](55,16)(55,-0)
\psline[linewidth=0.22](59,16)(59,-0)
\rput(49,13){$=$}
\rput(39,8){$\comonoidd$}
\rput(35,18){$\comonoidd$}
\rput(7,8){$\comonoidd$}
\rput(11,18){$\comonoidd$}
\rput(59,18){$\comontwo$}
\end{pspicture}


==> PIC/semigroup.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 20 23:27:29 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="42.5" y-min="3.12" y-max="22.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(22.5,10.62)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<ellipse p3= "(7.81,9.06)"
%	 p2= "(7.81,12.19)"
%	 p1= "(4.69,12.19)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(1.25,3.12);(1.25,3.12);(1.25,3.75);(1.25,3.75);(1.25,3.75);(1.25,5.62);
%	(1.25,5.62);(1.25,5.62);(5,9.38);(5,9.38)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(11.25,3.12);(11.25,3.12);(11.25,3.75);(11.25,3.75);(11.25,3.75);(11.25,5.62);
%	(11.25,5.62);(11.25,5.62);(7.5,9.38);(7.5,9.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(14.06,15.31)"
%	 p2= "(14.06,18.44)"
%	 p1= "(10.94,18.44)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(4.38,8.75);(4.38,8.75);(5.62,10);(5.62,10);(5.62,10);(7.5,11.88);
%	(7.5,11.88);(7.5,11.88);(11.25,15.62);(11.25,15.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(12.5,18.12);(12.5,18.12);(12.5,15.62);(12.5,15.62);(12.5,15.62);(12.5,18.12);
%	(12.5,18.12);(12.5,18.12);(12.5,22.5);(12.5,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(17.5,3.75);(17.5,3.75);(17.5,10);(17.5,10);(17.5,10);(17.5,11.88);
%	(17.5,11.88);(17.5,11.88);(13.75,15.62);(13.75,15.62)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(39.06,9.06)"
%	 p2= "(39.06,12.19)"
%	 p1= "(35.94,12.19)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(32.5,3.75);(32.5,3.75);(32.5,3.75);(32.5,3.75);(32.5,3.75);(32.5,5.62);
%	(32.5,5.62);(32.5,5.62);(36.25,9.38);(36.25,9.38)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(42.5,3.75);(42.5,3.75);(42.5,3.75);(42.5,3.75);(42.5,3.75);(42.5,5.62);
%	(42.5,5.62);(42.5,5.62);(38.75,9.38);(38.75,9.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(33.12,15)"
%	 p2= "(33.12,18.12)"
%	 p1= "(30,18.12)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(37.5,11.25);(37.5,11.25);(37.5,11.25);(37.5,11.25);(37.5,11.25);(36.25,11.88);
%	(36.25,11.88);(36.25,11.88);(32.5,15.62);(32.5,15.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(26.88,3.75);(26.88,3.75);(26.88,6.25);(26.88,6.25);(26.88,6.25);(26.88,11.88);
%	(26.88,11.88);(26.88,11.88);(30.62,15.62);(30.62,15.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(31.25,17.5);(31.25,17.5);(31.25,15.62);(31.25,15.62);(31.25,15.62);(31.25,17.5);
%	(31.25,17.5);(31.25,17.5);(31.25,22.5);(31.25,22.5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(42.5,22.5)
\rput(22.5,10.62){$=$}
\rput{0}(6.25,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline{->}(1.25,3.12)
(1.25,3.75)
(1.25,5.62)(5,9.38)
\psline{->}(11.25,3.12)
(11.25,3.75)
(11.25,5.62)(7.5,9.38)
\rput{0}(12.5,16.88){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline{->}(4.38,8.75)
(5.62,10)
(7.5,11.88)(11.25,15.62)
\psline{->}(12.5,18.12)
(12.5,15.62)
(12.5,18.12)(12.5,22.5)
\psline{->}(17.5,3.75)
(17.5,10)
(17.5,11.88)(13.75,15.62)
\rput{0}(37.5,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\pscustom[]{\psbezier{-}(32.5,3.75)(32.5,3.75)(32.5,3.75)(32.5,3.75)
\psline(32.5,3.75)(32.5,5.62)
\psline{->}(32.5,5.62)(36.25,9.38)
}
\pscustom[]{\psbezier{-}(42.5,3.75)(42.5,3.75)(42.5,3.75)(42.5,3.75)
\psline(42.5,3.75)(42.5,5.62)
\psline{->}(42.5,5.62)(38.75,9.38)
}
\rput{0}(31.56,16.56){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\pscustom[]{\psbezier{-}(37.5,11.25)(37.5,11.25)(37.5,11.25)(37.5,11.25)
\psline(37.5,11.25)(36.25,11.88)
\psline{->}(36.25,11.88)(32.5,15.62)
}
\psline{->}(26.88,3.75)
(26.88,6.25)
(26.88,11.88)(30.62,15.62)
\psline{->}(31.25,17.5)
(31.25,15.62)
(31.25,17.5)(31.25,22.5)
\end{pspicture}


==> PIC/seq-comp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 17:09:29 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="10" y-min="-14.38" y-max="16.25" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-14.38);(5,-14.38);(5,-8.12);(5,-8.12)"
%	 />
%<parallelogram p3= "(8,-8.12)"
%	 p2= "(8,-2.12)"
%	 fill-style= "none"
%	 p1= "(2,-2.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-2.12);(5,-2.12);(5,3.75);(5,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-5.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,6.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(10,3.88)"
%	 p2= "(10,9.38)"
%	 fill-style= "none"
%	 p1= "(0,9.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,9.38);(5,9.38);(5,16.25);(5,16.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,16.25)
\psline{->}(5,-14.38)(5,-8.12)
\pspolygon[](2,-2.12)(8,-2.12)(8,-8.12)(2,-8.12)
\psline{->}(5,-2.12)(5,3.75)
\rput(5,-5.12){$\ahh$}
\rput(5,6.88){$\aah$}
\pspolygon[](0,9.38)(10,9.38)(10,3.88)(0,3.88)
\psline{->}(5,9.38)(5,16.25)
\end{pspicture}


==> PIC/squares.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 25 15:39:53 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="130.62" y-min="-1.25" y-max="35.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(35,32.5);(35,32.5);(12.5,32.5);(12.5,32.5)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(36.88,2.5);(36.88,2.5);(12.5,2.5);(12.5,2.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,29.38);(5,29.38);(5,6.88);(5,6.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45.62,29.38);(45.62,29.38);(45.62,6.88);(45.62,6.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45.62,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.75,35.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.75,-0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,18.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46.89,18.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.75,31.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(118.75,31.88);(118.75,31.88);(96.25,31.88);(96.25,31.88)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(116.25,1.88);(116.25,1.88);(98.75,1.88);(98.75,1.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(88.75,28.76);(88.75,28.76);(88.75,6.25);(88.75,6.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(129.38,28.76);(129.38,28.76);(129.38,6.25);(129.38,6.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.75,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownThree$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(130.62,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownFour$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,18.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eight$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(130,18.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nine$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(107.5,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ten$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(129.38,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpThree$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(106.88,35.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seven$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130.62,35.62)
\rput(5,32.5){$\UpOne$}
\rput(45.62,32.5){$\UpTwo$}
\rput(5,2.5){$\DownOne$}
\psline{<-}(35,32.5)(12.5,32.5)
\psline{<-}(36.88,2.5)(12.5,2.5)
\psline{->}(5,29.38)(5,6.88)
\psline{->}(45.62,29.38)(45.62,6.88)
\rput(45.62,2.5){$\DownTwo$}
\rput(23.75,35.62){$\three$}
\rput(23.75,-0.62){$\four$}
\rput[r](3.75,18.12){$\five$}
\rput[l](46.89,18.12){$\six$}
\rput(88.75,31.88){$\UpOne$}
\psline{<-}(118.75,31.88)(96.25,31.88)
\psline{<-}(116.25,1.88)(98.75,1.88)
\psline{->}(88.75,28.76)(88.75,6.25)
\psline{->}(129.38,28.76)(129.38,6.25)
\rput(88.75,1.88){$\DownThree$}
\rput(130.62,1.88){$\DownFour$}
\rput[r](87.5,18.12){$\eight$}
\rput[l](130,18.12){$\nine$}
\rput(107.5,-1.25){$\ten$}
\rput(129.38,32.5){$\UpThree$}
\rput(106.88,35.62){$\seven$}
\end{pspicture}


==> PIC/string-diagrams <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 23 19:27:57 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-3.12" x-max="105" y-min="5" y-max="78.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,51.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(4,78)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,29.38);(5,29.38);(5,40.62);(5,40.62)"
%	 />
%<parallelogram p3= "(8,40.88)"
%	 p2= "(8,46.88)"
%	 p1= "(2,46.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,46.88);(5,46.88);(5,58.75);(5,58.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,43.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(8,59)"
%	 p2= "(8,65)"
%	 p1= "(2,65)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,65);(5,65);(5,75);(5,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,61.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(15.62,55.62);(15.62,55.62);(15.62,75);(15.62,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,29.38);(25,29.38);(25,40.62);(25,40.62)"
%	 />
%<parallelogram p3= "(28,40.62)"
%	 p2= "(28,46.62)"
%	 p1= "(22,46.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,46.88);(25,46.88);(25,75);(25,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,43.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,55.62);(11.88,55.62);(18.75,55.62);(18.75,55.62);(18.75,55.62);(15,49.38);
%	(15,49.38);(15,49.38);(11.88,55.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(33.12,34.06)"
%	 p2= "(33.12,69.69)"
%	 p1= "(-3.12,69.69)"
%	 stroke-width= "0.1"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(76.25,58.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.88,78)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.26,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(86.88,29.38);(86.88,29.38);(86.88,40.62);(86.88,40.62)"
%	 />
%<parallelogram p3= "(89.88,40.75)"
%	 p2= "(89.88,46.75)"
%	 p1= "(83.88,46.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.88,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(79.88,58.88)"
%	 p2= "(79.88,64.88)"
%	 p1= "(73.88,64.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(76.88,65);(76.88,65);(76.88,75);(76.88,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(76.88,61.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(87.5,73.75);(87.5,73.75);(87.5,75);(87.5,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.62,44.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(96.88,29.38);(96.88,29.38);(96.88,58.75);(96.88,58.75)"
%	 />
%<parallelogram p3= "(99.88,58.88)"
%	 p2= "(99.88,64.88)"
%	 p1= "(93.88,64.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(96.88,65);(96.88,65);(96.88,75);(96.88,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,61.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(72.5,46.86);(72.5,46.86);(79.38,46.86);(79.38,46.86);(79.38,46.86);(75.62,40.62);
%	(75.62,40.62);(75.62,40.62);(72.5,46.86)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.88,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75.62,46.88);(75.62,46.88);(75.62,48.12);(76.88,50);(78.12,51.88);(82.5,53.75);
%	(84.38,56.25);(86.25,58.75);(87.5,66.25);(87.5,69.38);(87.5,72.5);(87.5,74.38);
%	(87.5,74.38)"
%	 />
%<parallelogram p3= "(105,33.75)"
%	 p2= "(105,70)"
%	 p1= "(68.75,70)"
%	 stroke-width= "0.1"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(49.38,51.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lhsup$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lhsdown$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsmall$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\rhsup$
%</text>
%<multicurve fill-style= "none"
%	 points= "(86.88,46.88);(86.88,46.88);(86.25,49.38);(85.62,50.62);(85,51.88);(83.12,52.5);
%	(81.25,53.12);(79.38,53.75);(78.12,54.38);(77.5,55.62);(76.88,56.88);(76.88,58.75);
%	(76.88,58.75)"
%	 />
%<ellipse p3= "(81.87,52.1)"
%	 p2= "(81.88,54.38)"
%	 fill-color= "#ffffff"
%	 p1= "(79.38,54.38)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.75,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsmall$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80.62,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\simmetry$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(105,78.12)
\rput(1.88,51.88){$\bh$}
\rput(4,78){$\ch$}
\rput(14.38,78.12){$\chh$}
\rput(25,78.12){$\dh$}
\psline{->}(5,29.38)(5,40.62)
\pspolygon[](2,46.88)(8,46.88)(8,40.88)(2,40.88)
\psline{->}(5,46.88)(5,58.75)
\rput(5,43.75){$\af$}
\pspolygon[](2,65)(8,65)(8,59)(2,59)
\psline{->}(5,65)(5,75)
\rput(5,61.88){$\ag$}
\psline{->}(15.62,55.62)(15.62,75)
\rput(15,53.12){$\ak$}
\psline{->}(25,29.38)(25,40.62)
\pspolygon[](22,46.62)(28,46.62)(28,40.62)(22,40.62)
\psline{->}(25,46.88)(25,75)
\rput(25,43.75){$\ahh$}
\rput(25,26.25){$\aah$}
\pspolygon(11.88,55.62)
(18.75,55.62)
(15,49.38)(11.88,55.62)
\rput(5,26.25){$\aah$}
\pspolygon[linewidth=0.1](-3.12,69.69)(33.12,69.69)(33.12,34.06)(-3.12,34.06)
\rput[tr](76.25,58.12){$\bh$}
\rput(75.88,78){$\ch$}
\rput(86.26,78.12){$\chh$}
\rput(96.88,78.12){$\dh$}
\psline{->}(86.88,29.38)(86.88,40.62)
\pspolygon[](83.88,46.75)(89.88,46.75)(89.88,40.75)(83.88,40.75)
\rput(86.88,43.12){$\af$}
\pspolygon[](73.88,64.88)(79.88,64.88)(79.88,58.88)(73.88,58.88)
\psline{->}(76.88,65)(76.88,75)
\rput(76.88,61.88){$\ag$}
\psline{->}(87.5,73.75)(87.5,75)
\rput(75.62,44.38){$\ak$}
\psline{->}(96.88,29.38)(96.88,58.75)
\pspolygon[](93.88,64.88)(99.88,64.88)(99.88,58.88)(93.88,58.88)
\psline{->}(96.88,65)(96.88,75)
\rput(96.88,61.88){$\ahh$}
\rput(96.88,26.25){$\aah$}
\pspolygon(72.5,46.86)
(79.38,46.86)
(75.62,40.62)(72.5,46.86)
\rput(86.88,26.25){$\aah$}
\pscustom[]{\psbezier(75.62,46.88)(75.62,46.88)(75.62,48.12)(76.88,50)
\psbezier(78.12,51.88)(82.5,53.75)(84.38,56.25)
\psbezier(86.25,58.75)(87.5,66.25)(87.5,69.38)
\psbezier(87.5,72.5)(87.5,74.38)(87.5,74.38)
}
\pspolygon[linewidth=0.1](68.75,70)(105,70)(105,33.75)(68.75,33.75)
\rput(49.38,51.88){$\eqls$}
\rput(15,15){$\lhsup$}
\rput(15,5){$\lhsdown$}
\rput(15,10){$\eqlsmall$}
\rput(87.5,15){$\rhsup$}
\pscustom[]{\psbezier(86.88,46.88)(86.88,46.88)(86.25,49.38)(85.62,50.62)
\psbezier(85,51.88)(83.12,52.5)(81.25,53.12)
\psbezier(79.38,53.75)(78.12,54.38)(77.5,55.62)
\psbezier(76.88,56.88)(76.88,58.75)(76.88,58.75)
}
\rput{0.24}(80.62,53.24){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.25,-1.14)}
\rput(48.75,15){$\eqlsmall$}
\rput(80.62,53.12){$\simmetry$}
\end{pspicture}


==> PIC/string-diagrams.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 23 19:27:57 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-3.12" x-max="105" y-min="5" y-max="78.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,51.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(4,78)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,29.38);(5,29.38);(5,40.62);(5,40.62)"
%	 />
%<parallelogram p3= "(8,40.88)"
%	 p2= "(8,46.88)"
%	 p1= "(2,46.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,46.88);(5,46.88);(5,58.75);(5,58.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,43.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(8,59)"
%	 p2= "(8,65)"
%	 p1= "(2,65)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,65);(5,65);(5,75);(5,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,61.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(15.62,55.62);(15.62,55.62);(15.62,75);(15.62,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,29.38);(25,29.38);(25,40.62);(25,40.62)"
%	 />
%<parallelogram p3= "(28,40.62)"
%	 p2= "(28,46.62)"
%	 p1= "(22,46.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,46.88);(25,46.88);(25,75);(25,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,43.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,55.62);(11.88,55.62);(18.75,55.62);(18.75,55.62);(18.75,55.62);(15,49.38);
%	(15,49.38);(15,49.38);(11.88,55.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(33.12,34.06)"
%	 p2= "(33.12,69.69)"
%	 p1= "(-3.12,69.69)"
%	 stroke-width= "0.1"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(76.25,58.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.88,78)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.26,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,78.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(86.88,29.38);(86.88,29.38);(86.88,40.62);(86.88,40.62)"
%	 />
%<parallelogram p3= "(89.88,40.75)"
%	 p2= "(89.88,46.75)"
%	 p1= "(83.88,46.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.88,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(79.88,58.88)"
%	 p2= "(79.88,64.88)"
%	 p1= "(73.88,64.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(76.88,65);(76.88,65);(76.88,75);(76.88,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(76.88,61.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(87.5,73.75);(87.5,73.75);(87.5,75);(87.5,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.62,44.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(96.88,29.38);(96.88,29.38);(96.88,58.75);(96.88,58.75)"
%	 />
%<parallelogram p3= "(99.88,58.88)"
%	 p2= "(99.88,64.88)"
%	 p1= "(93.88,64.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(96.88,65);(96.88,65);(96.88,75);(96.88,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,61.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(72.5,46.86);(72.5,46.86);(79.38,46.86);(79.38,46.86);(79.38,46.86);(75.62,40.62);
%	(75.62,40.62);(75.62,40.62);(72.5,46.86)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.88,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75.62,46.88);(75.62,46.88);(75.62,48.12);(76.88,50);(78.12,51.88);(82.5,53.75);
%	(84.38,56.25);(86.25,58.75);(87.5,66.25);(87.5,69.38);(87.5,72.5);(87.5,74.38);
%	(87.5,74.38)"
%	 />
%<parallelogram p3= "(105,33.75)"
%	 p2= "(105,70)"
%	 p1= "(68.75,70)"
%	 stroke-width= "0.1"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(49.38,51.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lhsup$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lhsdown$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsmall$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\rhsup$
%</text>
%<multicurve fill-style= "none"
%	 points= "(86.88,46.88);(86.88,46.88);(86.25,49.38);(85.62,50.62);(85,51.88);(83.12,52.5);
%	(81.25,53.12);(79.38,53.75);(78.12,54.38);(77.5,55.62);(76.88,56.88);(76.88,58.75);
%	(76.88,58.75)"
%	 />
%<ellipse p3= "(81.87,52.1)"
%	 p2= "(81.88,54.38)"
%	 fill-color= "#ffffff"
%	 p1= "(79.38,54.38)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.75,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsmall$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80.62,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\simmetry$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(105,78.12)
\rput(1.88,51.88){$\bh$}
\rput(4,78){$\ch$}
\rput(14.38,78.12){$\chh$}
\rput(25,78.12){$\dh$}
\psline{->}(5,29.38)(5,40.62)
\pspolygon[](2,46.88)(8,46.88)(8,40.88)(2,40.88)
\psline{->}(5,46.88)(5,58.75)
\rput(5,43.75){$\af$}
\pspolygon[](2,65)(8,65)(8,59)(2,59)
\psline{->}(5,65)(5,75)
\rput(5,61.88){$\ag$}
\psline{->}(15.62,55.62)(15.62,75)
\rput(15,53.12){$\ak$}
\psline{->}(25,29.38)(25,40.62)
\pspolygon[](22,46.62)(28,46.62)(28,40.62)(22,40.62)
\psline{->}(25,46.88)(25,75)
\rput(25,43.75){$\ahh$}
\rput(25,26.25){$\aah$}
\pspolygon(11.88,55.62)
(18.75,55.62)
(15,49.38)(11.88,55.62)
\rput(5,26.25){$\aah$}
\pspolygon[linewidth=0.1](-3.12,69.69)(33.12,69.69)(33.12,34.06)(-3.12,34.06)
\rput[tr](76.25,58.12){$\bh$}
\rput(75.88,78){$\ch$}
\rput(86.26,78.12){$\chh$}
\rput(96.88,78.12){$\dh$}
\psline{->}(86.88,29.38)(86.88,40.62)
\pspolygon[](83.88,46.75)(89.88,46.75)(89.88,40.75)(83.88,40.75)
\rput(86.88,43.12){$\af$}
\pspolygon[](73.88,64.88)(79.88,64.88)(79.88,58.88)(73.88,58.88)
\psline{->}(76.88,65)(76.88,75)
\rput(76.88,61.88){$\ag$}
\psline{->}(87.5,73.75)(87.5,75)
\rput(75.62,44.38){$\ak$}
\psline{->}(96.88,29.38)(96.88,58.75)
\pspolygon[](93.88,64.88)(99.88,64.88)(99.88,58.88)(93.88,58.88)
\psline{->}(96.88,65)(96.88,75)
\rput(96.88,61.88){$\ahh$}
\rput(96.88,26.25){$\aah$}
\pspolygon(72.5,46.86)
(79.38,46.86)
(75.62,40.62)(72.5,46.86)
\rput(86.88,26.25){$\aah$}
\pscustom[]{\psbezier(75.62,46.88)(75.62,46.88)(75.62,48.12)(76.88,50)
\psbezier(78.12,51.88)(82.5,53.75)(84.38,56.25)
\psbezier(86.25,58.75)(87.5,66.25)(87.5,69.38)
\psbezier(87.5,72.5)(87.5,74.38)(87.5,74.38)
}
\pspolygon[linewidth=0.1](68.75,70)(105,70)(105,33.75)(68.75,33.75)
\rput(49.38,51.88){$\eqls$}
\rput(15,15){$\lhsup$}
\rput(15,5){$\lhsdown$}
\rput(15,10){$\eqlsmall$}
\rput(87.5,15){$\rhsup$}
\pscustom[]{\psbezier(86.88,46.88)(86.88,46.88)(86.25,49.38)(85.62,50.62)
\psbezier(85,51.88)(83.12,52.5)(81.25,53.12)
\psbezier(79.38,53.75)(78.12,54.38)(77.5,55.62)
\psbezier(76.88,56.88)(76.88,58.75)(76.88,58.75)
}
\rput{0.24}(80.62,53.24){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.25,-1.14)}
\rput(48.75,15){$\eqlsmall$}
\rput(80.62,53.12){$\simmetry$}
\end{pspicture}


==> PIC/tk-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 20 07:18:43 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="35" y-min="-20" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(21.88,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.62,-20)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(15.62,4.38);(15.62,4.38);(24.38,4.38);(24.38,4.38);(24.38,4.38);(24.38,-4.38);
%	(24.38,-4.38);(24.38,-4.38);(23.74,-3.77);(23.74,-3.77);(23.74,-3.77);(15.62,4.38);
%	(15.62,4.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(16.56,10.94)"
%	 p2= "(16.56,17.81)"
%	 p1= "(9.68,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "none"
%	 angle-start= "0"
%	 />
%<multicurve left-arrow= "head"
%	 points= "(15.62,11.87);(15.62,11.87);(20,7.5);(20,7.5);(20,7.5);(20,4.38);
%	(20,4.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,14.37)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\order$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(13.12,18.13);(13.12,18.13);(13.12,22.5);(13.12,22.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Tval$
%</text>
%<multicurve left-arrow= "head"
%	 points= "(10.62,11.89);(10.62,11.89);(6.25,7.5);(6.25,7.5);(6.25,7.5);(6.25,3.12);
%	(6.25,3.12)"
%	 fill-style= "none"
%	 />
%<multicurve left-arrow= "head"
%	 points= "(20.01,-0);(20.01,-0);(20,-6.25);(20,-6.25);(20,-6.25);(15.62,-10.62);
%	(15.62,-10.62)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(17.11,-12.11)"
%	 p2= "(17.11,-9.14)"
%	 p1= "(14.14,-9.14)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(15.62,-17.5);(15.62,-17.5);(15.62,-11.87);(15.62,-11.87)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,-20)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(3.75,-16.88);(3.75,-16.88);(3.75,-3.12);(3.75,-3.12)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve points= "(1.25,8.12);(1.25,8.12);(11.88,-2.5);(11.88,-2.5);(11.88,-2.5);(7.5,-6.88);
%	(7.5,-6.88);(7.5,-6.88);(1.25,-0.62);(1.25,-0.62);(1.25,-0.62);(1.25,8.12);
%	(1.25,8.12)"
%	 fill-style= "none"
%	 />
%<multicurve left-arrow= "head"
%	 points= "(10,-5);(10,-5);(15,-10);(15,-10);(15,-10);(15,-10);
%	(15,-10);(15,-10);(15.62,-10.62);(15.62,-10.62)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQ$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,25)
\rput(21.88,1.25){$\ahh$}
\rput(15.62,-20){$\Lhh$}
\psline(15.62,4.38)
(24.38,4.38)
(24.38,-4.38)
(23.74,-3.77)(15.62,4.38)
\rput{0}(13.12,14.38){\psellipse[](0,0)(3.44,-3.44)}
\psline{<-}(15.62,11.87)
(20,7.5)(20,4.38)
\rput(13.12,14.37){$\order$}
\psline{->}(13.12,18.13)(13.12,22.5)
\rput(13.12,25){$\Tval$}
\psline{<-}(10.62,11.89)
(6.25,7.5)(6.25,3.12)
\psline{<-}(20.01,-0)
(20,-6.25)(15.62,-10.62)
\rput{0}(15.62,-10.62){\psellipse[fillstyle=solid](0,0)(1.48,-1.48)}
\psline{->}(15.62,-17.5)(15.62,-11.87)
\rput(3.75,-20){$\dh$}
\psline{->}(3.75,-16.88)(3.75,-3.12)
\rput(5,0){$\shh$}
\psline(1.25,8.12)
(11.88,-2.5)
(7.5,-6.88)
(1.25,-0.62)(1.25,8.12)
\pscustom[]{\psline{<-}(10,-5)(15,-10)
\psbezier(15,-10)(15,-10)(15,-10)
\psline{-}(15,-10)(15.62,-10.62)
}
\rput(35,0){$\EQ$}
\end{pspicture}


==> PIC/two-one-appl.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:36:29 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.88" x-max="14.38" y-min="-11.88" y-max="13.75" auto-bounding="true">
%<parallelogram p3= "(14.38,-1.75)"
%	 p2= "(14.38,4.25)"
%	 p1= "(-1.88,4.25)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6.25,4.38);(6.25,4.38);(6.25,11.38);(6.25,11.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11.25,-8.75);(11.25,-8.75);(11.25,-1.75);(11.25,-1.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,-10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.25,-6.25);(1.25,-6.25);(1.25,-1.88);(1.25,-1.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.25,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-1.25,-6.25);(-1.25,-6.25);(3.75,-6.25);(3.75,-6.25);(3.75,-6.25);(1.26,-11.88);
%	(1.26,-11.88);(1.26,-11.88);(-1.25,-6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(14.38,13.75)
\pspolygon[](-1.88,4.25)(14.38,4.25)(14.38,-1.75)(-1.88,-1.75)
\psline{->}(6.25,4.38)(6.25,11.38)
\rput(6.25,1.25){$\ahh$}
\psline{->}(11.25,-8.75)(11.25,-1.75)
\rput(11.25,-10.62){$\eh$}
\rput(6.25,13.75){$\fh$}
\psline{->}(1.25,-6.25)(1.25,-1.88)
\rput(1.25,-8.75){$\aah$}
\pspolygon(-1.25,-6.25)
(3.75,-6.25)
(1.26,-11.88)(-1.25,-6.25)
\end{pspicture}


==> PIC/two-one.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 08 16:34:06 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.88" x-max="11.88" y-min="-10.62" y-max="13.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.25,-10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.25,-8.75);(1.25,-8.75);(1.25,-1.75);(1.25,-1.75)"
%	 />
%<parallelogram p3= "(11.88,-1.75)"
%	 p2= "(11.88,4.25)"
%	 fill-style= "none"
%	 p1= "(-1.88,4.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,4.38);(5,4.38);(5,12);(5,12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-8.75);(8.12,-8.75);(8.12,-1.75);(8.12,-1.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,-10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11.88,13.75)
\rput(1.25,-10.62){$\dh$}
\psline{->}(1.25,-8.75)(1.25,-1.75)
\pspolygon[](-1.88,4.25)(11.88,4.25)(11.88,-1.75)(-1.88,-1.75)
\psline{->}(5,4.38)(5,12)
\rput(5,1.25){$\ahh$}
\psline{->}(8.12,-8.75)(8.12,-1.75)
\rput(8.12,-10.62){$\eh$}
\rput(5,13.75){$\fh$}
\end{pspicture}


==> PIC/uni-cx-f.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Aug 25 12:03:52 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2" x-max="8.12" y-min="-11.25" y-max="22.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-8.25);(5,-8.25);(5,-1.25);(5,-1.25)"
%	 />
%<parallelogram p3= "(8,-1.25)"
%	 p2= "(8,4.75)"
%	 p1= "(2,4.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5.12,4.75);(5.12,4.75);(5,9.38);(5,9.38)"
%	 />
%<parallelogram p3= "(8.12,9.5)"
%	 p2= "(8.12,15.5)"
%	 p1= "(2.38,15.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,15.62);(5,15.62);(5,20.62);(5,20.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.12,-11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(8.12,22.5)
\psline{->}(5,-8.25)(5,-1.25)
\pspolygon[](2,4.75)(8,4.75)(8,-1.25)(2,-1.25)
\rput(5,1.88){$\aah$}
\rput(5,22.5){$\dh$}
\psline{->}(5.12,4.75)(5,9.38)
\pspolygon[](2.38,15.5)(8.12,15.5)(8.12,9.5)(2.38,9.5)
\psline{->}(5,15.62)(5,20.62)
\rput(5.12,-11.25){$\bhh$}
\rput(5,12.5){$\bbh$}
\end{pspicture}


==> PIC/uni-cx-p.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Aug 25 09:17:51 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2" x-max="20" y-min="-11.88" y-max="22.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(20,-1.25)"
%	 p2= "(20,4.75)"
%	 p1= "(2,4.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16,1.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,-8.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,-8.25);(17,-8.25);(17,-1.25);(17,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(17,-11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,-6.25);(2.5,-6.25);(7.5,-6.25);(7.5,-6.25);(7.5,-6.25);(5.01,-11.88);
%	(5.01,-11.88);(5.01,-11.88);(2.5,-6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,3.12);(3.75,3.12);(6.25,3.12);(6.25,3.12);(6.25,3.12);(5,0.62);
%	(5,0.62);(5,0.62);(3.75,3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,5);(16.88,5);(16.88,9.38);(16.88,9.38)"
%	 />
%<parallelogram p3= "(20,9.5)"
%	 p2= "(20,15.5)"
%	 p1= "(14.25,15.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,15.62);(16.88,15.62);(16.88,20.62);(16.88,20.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,22.5)
\psline{->}(5,-6.25)(5,0.75)
\pspolygon[](2,4.75)(20,4.75)(20,-1.25)(2,-1.25)
\rput(16,1.75){$\ahh$}
\rput(5,-8.12){$\aah$}
\psline{->}(17,-8.25)(17,-1.25)
\rput(17,-11.25){$\bhh$}
\pspolygon(2.5,-6.25)
(7.5,-6.25)
(5.01,-11.88)(2.5,-6.25)
\pspolygon(3.75,3.12)
(6.25,3.12)
(5,0.62)(3.75,3.12)
\rput(16.88,22.5){$\dh$}
\psline{->}(16.88,5)(16.88,9.38)
\pspolygon[](14.25,15.5)(20,15.5)(20,9.5)(14.25,9.5)
\psline{->}(16.88,15.62)(16.88,20.62)
\rput(16.88,12.5){$\bbh$}
\end{pspicture}


==> PIC/uni-eval-p-box.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 12:47:35 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2" x-max="20" y-min="-20" y-max="13.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-3.75);(5,-3.75);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(20,-1.25)"
%	 p2= "(20,4.75)"
%	 p1= "(2,4.75)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,4.75);(17,4.75);(17,11.75);(17,11.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16,1.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,-8.25);(17,-8.25);(17,-1.25);(17,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17,-11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<parallelogram p3= "(7.62,-9.62)"
%	 p2= "(7.62,-4.12)"
%	 p1= "(2.38,-4.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-14.38);(5,-14.38);(5,-9.88);(5,-9.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-6.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.75,3.12);(3.75,3.12);(6.25,3.12);(6.25,3.12);(6.25,3.12);(5,0.62);
%	(5,0.62);(5,0.62);(3.75,3.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,-14.38);(2.5,-14.38);(7.5,-14.38);(7.5,-14.38);(7.5,-14.38);(5.01,-20);
%	(5.01,-20);(5.01,-20);(2.5,-14.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,13.75)
\rput(17,13.75){$\dh$}
\psline{->}(5,-3.75)(5,0.75)
\pspolygon[](2,4.75)(20,4.75)(20,-1.25)(2,-1.25)
\psline{->}(17,4.75)(17,11.75)
\rput(16,1.75){$\ahh$}
\rput(5,-16.25){$\aah$}
\psline{->}(17,-8.25)(17,-1.25)
\rput(17,-11.25){$\bhh$}
\pspolygon[](2.38,-4.12)(7.62,-4.12)(7.62,-9.62)(2.38,-9.62)
\psline{->}(5,-14.38)(5,-9.88)
\rput(5,-6.88){$\chh$}
\pspolygon(3.75,3.12)
(6.25,3.12)
(5,0.62)(3.75,3.12)
\pspolygon(2.5,-14.38)
(7.5,-14.38)
(5.01,-20)(2.5,-14.38)
\end{pspicture}


==> PIC/uni-eval-p-old.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jan 16 09:46:55 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="18.75" y-min="-11.25" y-max="13.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,13.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(2.5,-2.5);(2.5,-2.5);(6.25,1.25);(6.25,1.25)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(13.12,4.38);(13.12,4.38);(13.12,11.88);(13.12,11.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.25,-3.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(13.12,-8.12);(13.12,-8.12);(13.12,-1.88);(13.12,-1.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,-11.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve points= "(-0.62,0.62);(-0.62,0.62);(5.62,-5.62);(5.62,-5.62);(5.62,-5.62);(-0.62,-5.62);
%	(-0.62,-5.62);(-0.62,-5.62);(-0.62,0.62)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(3.12,4.38);(3.12,4.38);(18.75,4.38);(18.75,4.38);(18.75,4.38);(18.75,-1.88);
%	(18.75,-1.88);(18.75,-1.88);(9.38,-1.88);(9.38,-1.88);(9.38,-1.88);(3.12,4.38);
%	(3.12,4.38)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(18.75,13.75)
\rput(13.12,13.75){$\dh$}
\psline{->}(2.5,-2.5)(6.25,1.25)
\psline{->}(13.12,4.38)(13.12,11.88)
\rput(13.12,1.25){$\ahh$}
\rput(1.25,-3.75){$\aah$}
\psline{->}(13.12,-8.12)(13.12,-1.88)
\rput(13.12,-11.25){$\bhh$}
\pspolygon(-0.62,0.62)
(5.62,-5.62)
(-0.62,-5.62)(-0.62,0.62)
\psline(3.12,4.38)
(18.75,4.38)
(18.75,-1.88)
(9.38,-1.88)(3.12,4.38)
\end{pspicture}


==> PIC/uni-eval-p-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 11:35:32 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="20" y-min="-13.12" y-max="13.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.62);(5,0.62)"
%	 />
%<parallelogram p3= "(20,-1.25)"
%	 p2= "(20,4.75)"
%	 p1= "(2,4.75)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,4.75);(17,4.75);(17,11.75);(17,11.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16,1.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,-8.25);(17,-8.25);(17,-1.25);(17,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17,-11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.25,-6.25);(1.25,-6.25);(8.12,-6.25);(8.12,-6.25);(8.12,-6.25);(4.38,-13.12);
%	(4.38,-13.12);(4.38,-13.12);(1.25,-6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,3.12);(3.75,3.12);(6.25,3.12);(6.25,3.12);(6.25,3.12);(5,0.62);
%	(5,0.62);(5,0.62);(3.75,3.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,13.75)
\rput(17,13.75){$\dh$}
\psline{->}(5,-6.25)(5,0.62)
\pspolygon[](2,4.75)(20,4.75)(20,-1.25)(2,-1.25)
\psline{->}(17,4.75)(17,11.75)
\rput(16,1.75){$\ahh$}
\rput(5,-8.12){$\aah$}
\psline{->}(17,-8.25)(17,-1.25)
\rput(17,-11.25){$\bhh$}
\pspolygon(1.25,-6.25)
(8.12,-6.25)
(4.38,-13.12)(1.25,-6.25)
\pspolygon(3.75,3.12)
(6.25,3.12)
(5,0.62)(3.75,3.12)
\end{pspicture}


==> PIC/uni-eval-s-g-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Feb 22 20:29:23 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.88" x-max="31.25" y-min="-16.25" y-max="18.75" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 points= "(2.5,-12.5);(2.5,-12.5);(2.5,-2.5);(2.5,-2.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(16.88,-2.5);(16.88,-2.5);(16.88,1.25);(16.88,1.25)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(14.38,-11.88);(14.38,-11.88);(14.38,-7.63);(14.38,-7.63)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,-16.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.62,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,-3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(26.88,-11.88);(26.88,-11.88);(26.88,-3.75);(26.88,-3.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(29.38,-16.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,-16.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(26.25,10);(26.25,10);(26.25,15.62);(26.25,15.62)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(-1.88,1.88);(-1.88,1.88);(7.5,-7.5);(7.5,-7.5);(7.5,-7.5);(21.88,-7.5);
%	(21.88,-7.5);(21.88,-7.5);(15.62,-1.25);(15.62,-1.25);(15.62,-1.25);(12.5,1.88);
%	(12.5,1.88);(12.5,1.88);(-1.88,1.88);(-1.88,1.88);(-1.88,1.88);(-1.88,1.88);
%	(-1.88,1.88);(-1.88,1.88);(-1.88,1.88);(-1.88,1.88)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(13.11,4.99);(13.11,4.99);(21.86,-3.76);(21.86,-3.76);(21.86,-3.76);(31.25,-3.75);
%	(31.25,-3.75);(31.25,-3.75);(31.25,9.99);(31.25,9.99);(31.25,9.99);(21.24,10);
%	(21.24,10);(21.24,10);(21.24,5);(21.24,5);(21.24,5);(15.62,5);
%	(15.62,5);(15.62,5);(13.11,4.99);(13.11,4.99)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(31.25,18.75)
\psline{->}(2.5,-12.5)(2.5,-2.5)
\psline{->}(16.88,-2.5)(16.88,1.25)
\psline{->}(14.38,-11.88)(14.38,-7.63)
\rput(14.38,-16.25){$\bhh$}
\rput(25.62,1.88){$\ahh$}
\rput(10,-3.12){$\shh$}
\psline{->}(26.88,-11.88)(26.88,-3.75)
\rput(29.38,-16.25){$\chh$}
\rput(2.5,-16.25){$\dh$}
\psline{->}(26.25,10)(26.25,15.62)
\rput(26.25,18.75){$\Lhh$}
\pscustom[]{\psline(-1.88,1.88)(7.5,-7.5)
\psline(7.5,-7.5)(21.88,-7.5)
\psline(21.88,-7.5)(15.62,-1.25)
\psline(15.62,-1.25)(12.5,1.88)
\psline(12.5,1.88)(-1.88,1.88)
\psbezier(-1.88,1.88)(-1.88,1.88)(-1.88,1.88)
\psbezier(-1.88,1.88)(-1.88,1.88)(-1.88,1.88)
}
\psline(13.11,4.99)
(21.86,-3.76)
(31.25,-3.75)
(31.25,9.99)
(21.24,10)
(21.24,5)
(15.62,5)(13.11,4.99)
\end{pspicture}


==> PIC/uni-eval-t-g.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 14 10:58:28 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5.62" x-max="30" y-min="-14.38" y-max="19.38" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 points= "(8.75,-11.88);(8.75,-11.88);(8.75,-3.25);(8.75,-3.25)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(15.62,-3.12);(15.62,-3.12);(20,1.25);(20,1.25)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(15.62,-11.88);(15.62,-11.88);(15.62,-6.38);(15.62,-6.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.62,-14.38)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.62,1.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,-3.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(26.25,-11.88);(26.25,-11.88);(26.25,-1.88);(26.25,-1.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,-14.38)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.75,-14.38)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(26.25,10.62);(26.25,10.62);(26.25,16.88);(26.25,16.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,19.38)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(5.62,0);(5.62,0);(13.12,0);(13.12,0);(13.12,0);(19.38,-6.25);
%	(19.38,-6.25);(19.38,-6.25);(11.88,-6.25);(11.88,-6.25);(11.88,-6.25);(5.62,0);
%	(5.62,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(16.88,4.38);(16.88,4.38);(23.12,-1.88);(23.12,-1.88);(23.12,-1.88);(30,-1.88);
%	(30,-1.88);(30,-1.88);(30,10.62);(30,10.62);(30,10.62);(22.5,10.62);
%	(22.5,10.62);(22.5,10.62);(22.5,4.38);(22.5,4.38);(22.5,4.38);(16.88,4.38);
%	(16.88,4.38);(16.88,4.38);(22.5,4.38);(22.5,4.38)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(30,19.38)
\psline{->}(8.75,-11.88)(8.75,-3.25)
\psline{->}(15.62,-3.12)(20,1.25)
\psline{->}(15.62,-11.88)(15.62,-6.38)
\rput(15.62,-14.38){$\bhh$}
\rput(25.62,1.88){$\ahh$}
\rput(13.12,-3.12){$\shh$}
\psline{->}(26.25,-11.88)(26.25,-1.88)
\rput(26.25,-14.38){$\chh$}
\rput(8.75,-14.38){$\dh$}
\psline{->}(26.25,10.62)(26.25,16.88)
\rput(26.25,19.38){$\Lhh$}
\psline(5.62,0)
(13.12,0)
(19.38,-6.25)
(11.88,-6.25)(5.62,0)
\psline(16.88,4.38)
(23.12,-1.88)
(30,-1.88)
(30,10.62)
(22.5,10.62)
(22.5,4.38)
(16.88,4.38)(22.5,4.38)
\end{pspicture}


==> PIC/uni-eval-u-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 18 02:29:00 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="25.62" y-min="-15.62" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(19.38,0.62)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(20.62,15);(20.62,15);(20.62,20.63);(20.62,20.63)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20.62,25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(15,-5.62);(15,-5.62);(25.62,-5.62);(25.62,-5.62);(25.62,-5.62);(25.62,-5);
%	(25.62,-5);(25.62,-5);(25.62,15);(25.62,15);(25.62,15);(15.62,15);
%	(15.62,15);(15.62,15);(15.62,4.38);(15.62,4.38);(15.62,4.38);(15.62,7.5);
%	(15.62,7.5);(15.62,7.5);(15.62,7.5);(15.62,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(3.75,-4.38);(3.75,-4.38);(8.13,-0.01);(8.13,-0.01)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(20,-11.25);(20,-11.25);(20,-5.76);(20,-5.76)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,-15.62)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,-8.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve points= "(3.75,4.38);(3.75,4.38);(13.75,-5.62);(13.75,-5.62);(13.75,-5.62);(25.62,-5.62);
%	(25.62,-5.62);(25.62,-5.62);(20,-5.62);(20,-5.62);(20,-5.62);(13.75,-5.62);
%	(13.75,-5.62);(13.75,-5.62);(3.75,4.38);(3.75,4.38);(3.75,4.38);(3.75,4.38);
%	(3.75,4.38);(3.75,4.38);(15.62,4.38);(15.62,4.38)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(25.62,25)
\rput(19.38,0.62){$\ahh$}
\psline{->}(20.62,15)(20.62,20.63)
\rput(20.62,25){$\Lhh$}
\pscustom[]{\psline(15,-5.62)(25.62,-5.62)
\psline(25.62,-5.62)(25.62,-5)
\psline(25.62,-5)(25.62,15)
\psline(25.62,15)(15.62,15)
\psline(15.62,15)(15.62,4.38)
\psline(15.62,4.38)(15.62,7.5)
\psbezier(15.62,7.5)(15.62,7.5)(15.62,7.5)
}
\psline{->}(3.75,-4.38)(8.13,-0.01)
\psline{->}(20,-11.25)(20,-5.76)
\rput(20,-15.62){$\bhh$}
\rput(1.88,-8.12){$\dh$}
\psline(3.75,4.38)
(13.75,-5.62)
(25.62,-5.62)
(20,-5.62)
(13.75,-5.62)
(3.75,4.38)
(3.75,4.38)(15.62,4.38)
\end{pspicture}


==> PIC/uni-eval-u-f-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 18 02:28:15 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="25.62" y-min="-15.62" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.12,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(20.62,14.99);(20.62,14.99);(20.62,20.62);(20.62,20.62)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20.62,25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(15,-5.62);(15,-5.62);(25.62,-5.62);(25.62,-5.62);(25.62,-5.62);(25.62,-5);
%	(25.62,-5);(25.62,-5);(25.62,15);(25.62,15);(25.62,15);(15.62,15);
%	(15.62,15);(15.62,15);(15.62,4.38);(15.62,4.38);(15.62,4.38);(15.62,7.5);
%	(15.62,7.5);(15.62,7.5);(15.62,7.5);(15.62,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(18.75,-11.11);(18.75,-11.11);(18.75,-5.62);(18.75,-5.62)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,-15.62)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve points= "(3.75,-5.62);(3.75,-5.62);(13.75,-5.62);(13.75,-5.62);(13.75,-5.62);(25.62,-5.62);
%	(25.62,-5.62);(25.62,-5.62);(20,-5.62);(20,-5.62);(20,-5.62);(13.75,-5.62);
%	(13.75,-5.62);(13.75,-5.62);(3.75,-5.62);(3.75,-5.62);(3.75,-5.62);(3.75,4.38);
%	(3.75,4.38);(3.75,4.38);(15.62,4.38);(15.62,4.38)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(25.62,25)
\rput(18.12,0){$\ahh$}
\psline{->}(20.62,14.99)(20.62,20.62)
\rput(20.62,25){$\Lhh$}
\pscustom[]{\psline(15,-5.62)(25.62,-5.62)
\psline(25.62,-5.62)(25.62,-5)
\psline(25.62,-5)(25.62,15)
\psline(25.62,15)(15.62,15)
\psline(15.62,15)(15.62,4.38)
\psline(15.62,4.38)(15.62,7.5)
\psbezier(15.62,7.5)(15.62,7.5)(15.62,7.5)
}
\psline{->}(18.75,-11.11)(18.75,-5.62)
\rput(18.75,-15.62){$\bhh$}
\psline(3.75,-5.62)
(13.75,-5.62)
(25.62,-5.62)
(20,-5.62)
(13.75,-5.62)
(3.75,-5.62)
(3.75,4.38)(15.62,4.38)
\end{pspicture}


==> PIC/uni-eval-u-g.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 14 11:13:41 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="9.38" y-min="-11.25" y-max="16.25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,-11.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.62,3.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(5,-8.75);(5,-8.75);(5,-3.12);(5,-3.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(5.62,7.5);(5.62,7.5);(5.62,14.38);(5.62,14.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.62,16.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(1.88,0);(1.88,0);(9.38,-7.5);(9.38,-7.5);(9.38,-7.5);(9.38,-7.5);
%	(9.38,-7.5);(9.38,-7.5);(9.38,7.5);(9.38,7.5);(9.38,7.5);(1.88,7.5);
%	(1.88,7.5);(1.88,7.5);(1.88,0);(1.88,0);(1.88,0);(1.88,0);
%	(1.88,0);(1.88,0);(1.88,7.5);(1.88,7.5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(9.38,16.25)
\rput(5,-11.25){$\dh$}
\rput(5.62,3.12){$\ahh$}
\psline{->}(5,-8.75)(5,-3.12)
\psline{->}(5.62,7.5)(5.62,14.38)
\rput(5.62,16.25){$\Lhh$}
\pscustom[]{\psline(1.88,0)(9.38,-7.5)
\psbezier(9.38,-7.5)(9.38,-7.5)(9.38,-7.5)
\psline(9.38,-7.5)(9.38,7.5)
\psline(9.38,7.5)(1.88,7.5)
\psline(1.88,7.5)(1.88,0)
\psbezier(1.88,0)(1.88,0)(1.88,0)
\psline(1.88,0)(1.88,7.5)
}
\end{pspicture}


==> PIC/uni-eval-uMN-g-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Feb 22 20:31:05 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="28.75" y-min="-10" y-max="20" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(4.38,-10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(4.38,-6.88);(4.38,-6.88);(4.38,1.88);(4.38,1.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 points= "(15,-6.88);(15,-6.88);(15,-2.5);(15,-2.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,-10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(23.12,-6.88);(23.12,-6.88);(23.12,-2.49);(23.12,-2.49)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.12,-10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 points= "(23.75,11.25);(23.75,11.25);(23.75,16.88);(23.75,16.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.75,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve points= "(0,6.25);(0,6.25);(8.75,-2.5);(8.75,-2.5);(8.75,-2.5);(28.75,-2.5);
%	(28.75,-2.5);(28.75,-2.5);(28.75,11.25);(28.75,11.25);(28.75,11.25);(18.75,11.25);
%	(18.75,11.25);(18.75,11.25);(18.75,6.25);(18.75,6.25);(18.75,6.25);(5.63,6.25);
%	(5.63,6.25);(5.63,6.25);(0,6.25);(0,6.25)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28.75,20)
\rput(4.38,-10){$\dh$}
\psline{->}(4.38,-6.88)(4.38,1.88)
\psline{->}(15,-6.88)(15,-2.5)
\rput(15,-10){$\bhh$}
\rput(16.25,2.5){$\ahh$}
\psline{->}(23.12,-6.88)(23.12,-2.49)
\rput(23.12,-10){$\chh$}
\psline{->}(23.75,11.25)(23.75,16.88)
\rput(23.75,20){$\Lhh$}
\psline(0,6.25)
(8.75,-2.5)
(28.75,-2.5)
(28.75,11.25)
(18.75,11.25)
(18.75,6.25)
(5.63,6.25)(0,6.25)
\end{pspicture}


==> PIC/uni-type-Ahh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:42:12 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="0" y-min="-5" y-max="10.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,-5);(0,-5);(0,10.62);(0,10.62)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(0,10.62)
\psline(0,-5)(0,10.62)
\end{pspicture}


==> PIC/uni-type-Phh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:36:01 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.62" x-max="6.25" y-min="-16.25" y-max="10" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0.62,-10.62);(0.62,-10.62);(0.62,10);(0.62,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,-11.25);(1.25,-11.25);(1.25,9.38);(1.25,9.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,-11.88);(1.88,-11.88);(1.88,8.75);(1.88,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,-14.38);(4.38,-14.38);(4.38,6.25);(4.38,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,-15);(5,-15);(5,5.62);(5,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\spce$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-15);(5,-15);(5,5.62);(5,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,-15.62);(5.62,-15.62);(5.62,5);(5.62,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,-15.62);(5.62,-15.62);(5.62,5);(5.62,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,-16.25);(6.25,-16.25);(6.25,4.38);(6.25,4.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(6.25,10)
\psline(0.62,-10.62)(0.62,10)
\psline(1.25,-11.25)(1.25,9.38)
\psline(1.88,-11.88)(1.88,8.75)
\psline(4.38,-14.38)(4.38,6.25)
\psline(5,-15)(5,5.62)
\rput(3.12,0){$\spce$}
\psline(5,-15)(5,5.62)
\psline(5.62,-15.62)(5.62,5)
\psline(5.62,-15.62)(5.62,5)
\psline(6.25,-16.25)(6.25,4.38)
\end{pspicture}


==> PIC/uni-type-Phhh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:45:40 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.62" x-max="6.88" y-min="-8.75" y-max="11.88" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0.62,-2.5);(0.62,-2.5);(0.62,11.88);(0.62,11.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\spce$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.25,-3.12);(1.25,-3.12);(1.25,11.25);(1.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,-3.75);(1.88,-3.75);(1.88,10.62);(1.88,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,-6.88);(5,-6.88);(5,7.5);(5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,-7.5);(5.62,-7.5);(5.62,6.88);(5.62,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,-8.12);(6.25,-8.12);(6.25,6.25);(6.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,-8.75);(6.88,-8.75);(6.88,5.62);(6.88,5.62)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(6.88,11.88)
\psline(0.62,-2.5)(0.62,11.88)
\rput(3.75,3.12){$\spce$}
\psline(1.25,-3.12)(1.25,11.25)
\psline(1.88,-3.75)(1.88,10.62)
\psline(5,-6.88)(5,7.5)
\psline(5.62,-7.5)(5.62,6.88)
\psline(6.25,-8.12)(6.25,6.25)
\psline(6.88,-8.75)(6.88,5.62)
\end{pspicture}


==> PIC/uni-type.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:33:19 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="31.88" y-min="-13.12" y-max="10.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,-10);(10,-10);(10,10.62);(10,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,-10.62);(25,-10.62);(25,10);(25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-11.25);(25.62,-11.25);(25.62,9.38);(25.62,9.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.25,-11.88);(26.25,-11.88);(26.25,8.75);(26.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.88,-12.5);(26.88,-12.5);(26.88,8.12);(26.88,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,-13.12);(27.5,-13.12);(27.5,7.5);(27.5,7.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Phh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(31.88,10.62)
\rput(5,0){$\Ah$}
\psline(10,-10)(10,10.62)
\rput(15,0){$\eqls$}
\psline(25,-10.62)(25,10)
\psline(25.62,-11.25)(25.62,9.38)
\psline(26.25,-11.88)(26.25,8.75)
\psline(26.88,-12.5)(26.88,8.12)
\psline(27.5,-13.12)(27.5,7.5)
\rput(31.88,0){$\Phh$}
\end{pspicture}

